CELLO: Co-designing Schedule and Hybrid Implicit/Explicit Buffer for Complex Tensor Reuse

Tensor algebra accelerators have been gaining popularity for running high-performance computing (HPC) workloads. Identifying optimal schedules for individual tensor operations and designing hardware to run these schedules is an active area of research. Unfortunately, operators in HPC workloads such as Conjugate Gradient often have operators with skewed shapes, fundamentally limiting the reuse any schedule can leverage. Moreover, the operators form a complex DAG of dependencies, making it challenging to apply simple fusion/pipelining techniques to extract inter-operation reuse. To address these challenges, this work proposes an accelerator CELLO. CELLO uses a novel on-chip buffer mechanism called CHORD co-designed with a novel scheduler called SCORE, which together enables identifying and exploiting reuse over complex DAGs of tensor operations. CELLO provides 4x geomean speedup and 4x energy efficiency over state-of-the-art accelerators across HPC workloads.

==> 01-Introduction-old-Apr8.tex <==
%\vspace{-3mm}
\section{Introduction}
\label{sec:introduction}


\begin{comment}
    Points to be made in the intro
        - High value GEMM workloads have complex dependencies []
        - Traditional pipelining does not respond well to these dependencies
        -Keeping operands on-chip is key to get a good performance.
                - Caches - Implicit and Workload agnostic + hardware overheads
                - Spads - Explicitly managed (large map-space and expensive search and buffer allocation)
                - CHORD: A hybrid implicit and explicit management, which is cycle-level implicit and coarse-grained explicit, so the cost lowers enough to manage the SRAM online..
        - SCORE: Fast scheduler for low intensity ops that deals with more complex dependencies, and also provides metadata to CHORD..
        - Skewed GEMMs can have surprisingly low arithmetic intensity??
        
    


    
\end{comment}





As Deep Learning (DL) emerged as a high-value workload, the computer architecture community responded by proposing custom accelerators for DNNs~\cite{eyeriss2016isca,kwon2018maeri,tpu-isca,nvdla}. 
The most common fundamental operation for these DNNs was matrix multiplication, often expanded from convolutional layers that were common in DNNs at that time. These GEMMs offered good reuse opportunities because of their large dimensions and relatively cubic aspect ratios, allowing early DNN accelerators to successfully schedule each layer independently and achieve maximum utilization for the networks they targeted at design-time.

%Furthermore, prior works have also looked at the accelerators for sparse tensor workloads~\cite{sigma,eie,extensor,eyeriss2} which eliminate irrelevant multiplications and memory accesses.}% Unfortunately, this approach lowers intensity even further, and straightforwardly applying these to CG on a GEMM-by-GEMM operation basis results in compute under-utilization due to limited memory bandwidth.


Recently, work like the Tensor Algebra COmplier (TACO) \cite{XXXTaco} has spurred research interest in generalized tensor applications, including sparse tensor algebra. %The computer architecture community has responded with recent proposals that generalize custom accelerators to efficiently target a superset of DNNs \cite{extensor, tensaurus, dave2020hardware, tensorlib, flextensor} namely, applications represented as arbitrary DAGs of \emph{tensor operations} and non-linearities for DL activation functions.
However, this generalization brings new challenges: tensor-algebra applications have diverse shapes, sparsity ratios, and dependency graphs. %Worse, this is coupled with a trend in DNNs away from large, monolithic GEMMs and towards numerous small independent matrix multiplications\footnote{Often called \emph{batched} GEMMs, which should not be confused with DNN batch size.} with less cubic aspect ratios.
This is significant because of an underappreciated fundamental property: namely, \textit{not all dense GEMMs with large number of multiplications are compute-bound even in the best case}. As shown in \autoref{fig:ai1}, a \emph{skewed} aspect ratio inherently decreases \emph{arithmetic intensity} (AI), thus making the GEMM memory-bound and leaving datapath resources idle. For example, to saturate its datapaths the TPU v3 and v4 architectures require an AI of approximately 150 and 250 respectively~\cite{tpuv4}.  %Sparse tensor algebra introduces similar challenges, as removing multiplication-by-zero decreases the AI numerator, while transferring \emph{metadata} for compression formats increases the denominator relatively.}

\insertFigureScaled{ai1}{Degradation of arithmetic intensity on two GEMMs with the same number of multiplications due to aspect ratio skew.\vspace{-3mm}}{.75}



%\insertFigure{no-fusion}{Pipelining cannot simply be applied to complex DAGs due to - 1) Delayed downstream dependency, 2) varying shapes, 3) consumers at multiple reuse distances 4) need to preserve layout across conusmers.\vspace{-3mm}}


%The reason for this is low arithmetic intensity for a skewed GEMM and it can be as low below 1 op/byte. Currently, most scheduling strategies optimize matrix multiplications independently and compose them to execute in an op-by-op manner, which leads to low performance in applications with skewed GEMMs.}

\begin{comment}
A real-world quantification of this phenomenon is captured by HPCG benchmark~\cite{dongarra2015hpcg,hpcg2021}, which runs Conjugate Gradient (CG)---a widely used HPC solver application represented as a DAG of tensor operations.

\input{tables/hpcg}

%\footnote{HPCG is a benchmark for supercomputers that runs CG. \MP{Footnote 1 adds no real information. Cut. }}
As \autoref{tables:hpcg} shows, CG achieves only 1-3\% of peak performance on top 7 supercomputers. 
Therefore, intra-operation reuse alone is not sufficient.
The overall throughput can be increased by improving the arithmetic intensity (i.e., on-chip data reuse), which can be done by seeking inter-operation reuse.
\end{comment}

Prior works have also shown that simple pipelining of adjacent operation~\cite{tileflow,isca-pip,yan2020hygcn} can enable some inter-operation reuse, but we demonstrate that this leaves out significant other sources of reuse, including complex cascade of tensors in case of delayed downstream consumers. It is also challenging to simply apply traditional inter-operation pipelining in cases of these dependencies, because of the delayed downstream dependencies, varying shapes of skewed GEMMs and multiple of these downstream consumers as~\autoref{fig:no-fusion} shows. %\TK{Fig 4 getting referenced before Fig 3, i suggest bring it before Fig 4 then} 
~\autoref{fig:dfg} shows an actual complex cascade of tensor operations found in CG, a high-value HPC workload rich in these complexities.
Thus, we need mechanisms to cache these intermediate tensors within SRAMs, since there are situations where simple pipelining cannot be applied.

DNN accelerators have previously used scratchpads because they have suited the energy and area needs of the accelerator. Prior works like buffets~\cite{buffets} make use of \emph{explicit decoupled data orchectration} where scratchpad RAM are supplemented by simple pointer and credit management scoreboarding. This is called explicit because data placement and RAM replacement are schedule-controlled, and decoupled because it operates on bulk-synchronous fills. These work well for executing one layer at a time, when all dimensions of matrices have sufficient reuse.
%While explicit orchestration works well for scheduling single matrix multiplication at a time, considering data placement, for inter-operation reuse statically in general tensor algebra is a diabolically hard problem. 
 In order to reuse such operands, specially where intra-operation reuse is simply not enough, storing these operands in the on-chip buffer is essential, and multiple of these operands contend for space inside the buffer. We show in~\autoref{sec:arguments} that the design-space to accommodate multiple tensors inside a buffer space explodes in complexity. ~\autoref{sec:arguments} also discusses why running statically known DAGs does not necessarily imply that scratchpads are not burdensome and don't have design-time overheads.
%Overall, the co-dependence on schedule, available scratchpad capacity and different downstream consumers make the explicit scheduling problem too challenging.

\insertFigure{no-fusion}{Pipelining cannot simply be applied to complex DAGs due to - 1) Delayed downstream dependency, 2) varying shapes, 3) consumers at multiple reuse distances 4) need to preserve layout across conusmers.\vspace{-3mm}}

Alternatively, caches are widespread on-chip storage structures that use \emph{implicit} data orchestration. Ideally, the presence of the cache is not architecturally exposed and the hardware itself does the best job possible of reusing the data. (In practice, best optimization is often made by cache-aware scheduling policies, blurring the line between implicit and explicit.) However, the area and energy overhead for tag matching make it less appealing for custom accelerators, as well as the possibility of increased misses due to conflicts. Overheads aside, cache policies typically operate at line granularity of unified address streams, rather than having higher-level knowledge of tensors, blocks, or intended reuse distance. This results in cache policies often rejecting the data that may have high reuse frequency (by virtue of reuse of the whole block) but might not be the immediate vicinity (i.e., high reuse distance).

To this end, we propose~\SpadNamenospace\footnote{\SpadNameexp}, a hybrid design that obtains DAG information from the workload but places elements of tensor implicitly in the buffer\footnote{We use "buffer" as an overarching term for on-chip SRAMs like cache, scratchpad, FIFOs etc.}. 
%~\SpadName is workload-aware, as it uses high-level metadata like starting and ending global address of a tensor, tensor-level reuse frequency and distance from the workload (the explicit component), but implicitly controls placement of elements of tensors without being burdensome to the programmer. ~%\TK{it might be worth adding a footnote saying you use scratchpad and buffer interchangeably in this paper} 
%\TK{based on what the footnote says its unclear whether chord is a scratchpad or cache }
~\SpadName has properties specifically chosen to supplement explicitly managed buffers that ease the scheduling problems while significantly reducing the area and energy overheads of traditional caches. Specifically,~\SpadName uses per-tensor replacement policies that can be configured by the schedule at coarse granularity.
%for operands with downstream consumers that uses implicit replacement at a tensor granularity rather than a line granularity. 
%In this work we propose two such policies- \\(1) \PolicyA - \SpadName is filled in the queue order and once the buffer is full, the spilling data is sent straight to the DRAM.\\
%(2) \PolicyBnospace\footnote{\PolicyBexp} - If the current tensor has a higher reuse frequency and lower reuse distance (in case of same frequency) than the previously written tensor, the current tensor starts replacing the previous tensor by the tail.
Because of its extremely coarsened granularity, ~\SpadName retains the benefit of a scratchpad over a cache (i.e., with minimal (<1\% of that of cache) tag matching overhead) 
%Hence it gets rid of caches' tag matching overhead and 
while
our proposed implicit tensor replacement policies~\PolicyA and \PolicyB remove the challenge of statically coming up with the data placement and replacement strategies statically for operands in multiple operations.

We also propose ~\DataflowNamenospace\footnote{\DataflowNameexp} a downstream dependency aware novel scheduling strategy. 
\DataflowName identifies the delayed downstream dependencies that require writeback from those where pipelining would work, and steers the tensors with delayed writeback dependencies to~\SpadNamenospace. In order to exploit the reuse on delayed downstream consumers, it is important to make sure that the order in which the elements are produced as same as the order in which they are consumed, otherwise, layout transformation is required. \DataflowName minimizes the need to transform the layout of the tensor (aka swizzle).%\TK{minimizing layout transformation is an important feature. Lets highlight it more explcitly. As in mention that the dataflow of the current op and downstream op may be different requiring expensive layout transformation, and SCORE tries to minimize that.}%It consists of the following steps - \\ 
%\TK{there seems to be some missing text here?}
%(1) Marking all the edges in the DAG of tensor operations with pipelining opportunities. This is useful in situations where tensors have delayed downstream consumers which can be visualized as a long edge in the DAG.\\
%(2) Assigning loop orders and tiling strategies to ensure that pipelining is actually exploited and layout transformation overhead of a tensor is minimized.\\
%\DataflowName reduces the contending tensors and also ensures minimum layout transformation (aka swizzling) which is also the motivation behind~\PolicyA policy.
%The main reason is the low arithmetic intensity achieved by the execution of Conjugate Gradient on CPUs/GPUs. 
%The main reason for this that the tensor multiplications---which we term \emph{operation} for this paper---%\MP{This definition is also too important to be in a footnote
 %used in CG have extremely unbalanced aspect ratios, which significantly lowers arithmetic intensity and data reuse.} %\MP{I feel like this point should come earlier, perhaps before the previous paragraph.}
%We use the term \emph{skewed} GEMMs to refer to such SpMMs/GEMMs---though notably, in the limit they can devolve to matrix-vector multiplication, i.e. if the shape of the matrix is 100,000:8.}%The main reason for this is costly data movement and communication between compute clusters/pods\MP{This explanation doesn't make sense either. Needs a reuse/intensity component. Even if this made sense, does GOGETA actually fix this problem?}.




%\TK{@Raveesh - I think we can move this para to para 3. Basically start with current para 2 on GEMMs, reuse and spatial accelerators. Then introduce CG. So intersperse this para with current para 3}


%making inter-operation reuse essential.

%This work explores inter-operation reuse opportunities for kernels like CG to enhance its arithmetic intensity.

%However, the~\GEMM in CG have orders of magnitude lower arithmetic intensity compared to SpMMs/GEMMs in DNNs and offer less reuse opportunities within one operation as~\autoref{fig:ai}~(\autoref{sec:ai}) discusses later in the paper. 
%Thus, executing CG at the granularity of a GEMM, reading tensors from DRAM and writing the output of each GEMM to DRAM, makes it highly memory bound leading to low compute utilization as~\autoref{\:hpcg} shows. 
\begin{comment}
Fusing \textit{adjacent} low AI matrix multiplication operators has recently been leveraged for applications like Graph Convolutional Networks (GCN)~\cite{garg2021understanding,yan2020hygcn,liang2020engn} and Transformers~\cite{flat,flashattention} 
wherein tiles of the intermediate tensor are manifested and consumed within the 
on-chip memory hierarchy in a \textit{pipelined} manner, reducing  intermediate output data movement to and from DRAM. We call this \emph{adjacent-op pipelining} in this work.
Other recent works have looked at enumerating the design-space for such adjacent-op pipelining~\cite{garg2021understanding} and 
%\TK{is this what the isca paper does?}\RG{Yep}
identifying optimal pipelined dataflow choices~\cite{isca-pip}, thereby enhancing better compute utilization when running memory-bound tensors.

While traditional adjacent-op pipelining is promising for DAGs with linear chains of operators (i.e., most DNNs today and GCNs), we show in this work that it is insufficient to capture nuances in more complex DAGs, such as those used in HPC kernels like CG.
Specifically, delayed downstream consumption of fanout of tensors, implies that traditional pipelining which overwrites the previously consumed tile cannot be applied directly due to a later dependency.%~\autoref{fig:no-fusion} shows an example, where tensor S has a delayed consumer.
 Moreover nuances such as data layouts of one tensor consumed in various operations is not captured by adjacent pipelining.
%that prior works cannot capture, as we discuss later. \autoref{table:related} enumerates this.

In this work, we coin the term \emph{generalized inter-operation reuse} to widen the scope of inter-operation reuse beyond adjacent operators to include additional reuse opportunities (\autoref{table:related}).
%as a wider generalization of traditional \emph{adjacent-operator pipelining}, introducing three additional reuse opportunities (\autoref{table:related}). 
We also propose \DataflowName (\TitleExpansion), which is a systematic strategy for mapping DAG of tensor operations exploiting the generalized inter-operation reuse opportunities, with the goal of enhancing the AI of the overall application.
%\DataflowName is applicable to any DAG of operations. 
We demonstrate that while \DataflowName is essential for extracting reuse in complex DAGs like CG, it can also be applied to simpler DAGs like GCNs and DNNs, thus preserving generalizability.

%\insertFigurePartnnnn{no-fusion}{A part of the CG tensor dependency graph where a node represents the equation in~\autoref{alg:cg_einsum} and edge represents the output of the source node equation. Please refer to ~\autoref{fig:dfg} for complete graph of CG.\vspace{-3mm}}%\RG{contraction heavy}}
\end{comment}

We summarize our contributions below:
%\TK{I think the contribitions can be listed more succinctly. I would suggest each contribution bullet pointing to a specific section of paper. }

\squishlist
\item We characterize the challenge of skewed GEMMs/SpMMs in tensor-algebra applications and the challenges of generalizing traditional inter-operation pipelining~\footnote{Not to be confused with inter-operation "reuse" since pipelining is a narrow aspect of inter-operation reuse}. (\autoref{sec:ai}).
%We also observe that these patterns are frequent across other HPC workloads which we discuss in ~\autoref{sec:background}.
%\item We propose a systematic methodology to formulate the data reuse opportunities in an arbitrary DAG of tensor operations and based on the reuse opportunities, we derive the loop orders and tile sizes.(\autoref{sec:dataflows}).
%\item We co-optimize the loop orders and tiling strategies for the GEMM operations in order to leverage reuse from both traditional inter-operation pipelining and distance based inter-operation reuse.
\item We propose~\SpadName(\autoref{sec:chorus}), a buffer structure for operands with downstream consumers that uses tensor-operand level replacement, that reduces tag match overhead and considers a more wholistic view of the object rather than a cache line. Cycle-level implicit tensor level replacement also eases the burden of solving tensor allocation involving multiple tensors statically which is a hard problem. 
\item We propose~\DataflowName (\autoref{sec:score}), a scheduler which identifies the operands with delayed dependencies that require writeback (and hence \SpadNamenospace), and proposes a schedule that maximizes inter-operation reuse and minimizes the layout transformation of the operands across different consumers.

%\item %Prior works on pipelining~\cite{flat,tangram,garg2021understanding,yan2020hygcn} divide the whole compute region into contiguous chunks and an operation is mapped on to a chunk as~\autoref{fig:spacetime} (top sub-figure) shows.\TK{seems odd to cite Fig 12 in intro}
%However, there is not much reuse within a single operation and the whole tensor needs to be communicated between the chunks. 
%\TK{this seems like a very specific optimization - and confusing here about what is lower BW vs higher BW NoC .. in fact i dont recall our arch section / Table IV talking about two NoCs with diff BWs? cant you state this contribution more generally about a communication BW optimized scalable inter-operation tiling strategy?}
%We propose a scalable inter-operation tiling strategy that reduces inter-cluster communication(~\autoref{sec:tiling}).  %a mapping that reduces memory accesses and communication at the tensor dependency graph level.
%\end{itemize}
%\item We propose buffer management schemes that reuse initial tiles of the output and can also replace the tensor based on future reuse distance and frequency~(\autoref{sec:tornado}). %the notion of Tensor-operand level reuse distance for such patterns and a tensor organization strategy inside the buffer hierarchy (\autoref{sec:tornado}).

\item We demonstrate the limitations of caches, namely, area overhead and line-level policies and the limitations of scratchpad, namely complexities in static buffer allocation of multiple delayed downstream consumers (\autoref{sec:arguments}).

\item \SpadName and \DataflowName are generally applicable to diverse tensor applications as it applies to all DAGs and achieve 2.51x geomean speedup and 4x improvement in energy efficiency across all workloads evaluated (\autoref{sec:eval}).

%\item \reviewme{ } 
%\item We propose a novel data orchestration technique \DataflowName which allows for efficient replacement, placement and prefetching of data for applications with variable reuse distance patterns. Since reuse distance is a generalization, \DataflowName can be used for applications with only intra-operation reuse and inter-operation pipelining opportunities as well.
%\item We propose a novel buffer idiom \TODO{name} which improves performance and energy over caches and scratchpads by \TODO{xx} and \TODO{xx}
\squishend

\begin{comment}
\emph{Inter-operation pipelining (aka fusion)} has been shown to be beneficial for accelerators for applications like Graph Neural Networks~\cite{garg2021understanding,yan2020hygcn,liang2020engn} where the intermediate tensor is reused between an SpMM and a GEMM,  reducing  intermediate output data movement to and from DRAM.
It has been shown that this approach is more challenging~\cite{dnnfusion,flat} and has a larger design-space~\cite{garg2021understanding} than straightforward element-wise fusion done by ML compilers today, for example, matrix-multiplication and ReLU fusion.
%Unfortunately, \textit{traditional inter-operation pipelining} often consumes the intermediate data and does not keep it in the memory. 
%Traditionally, \textit{inter-operation pipelining} has been exploited in prior works~\cite{tangram,garg2021understanding,yan2020hygcn,flat} %across various application domains 
%to reduce the data movement to DRAM, by consuming the portion of the tensor as it is produced 
\TK{I think we need to transition to saying that inter-operation pipelining does not capture all inter-operation reuse opportunities as this work identifies.}
Unfortunately, the additional complexity of inter-operation dependency graphs in certain applications introduces additional challenges which confounds the attempts at \emph{traditional inter-operation pipelining.} Furthermore, just capturing reuse in adjacent operations misses the overall opportunity to consider future instances of reuse of tensors in the entire program. \reviewme{We use CG as an example to discuss these challenges and missed opportunities:}

(1) Operations can have a delayed downstream consumer. Therefore, the data must remain resident in the memory hierarchy. However, traditional pipelining overwrites tiles that are consumed by the adjacent operation.
%~\autoref{fig:dfg} shows CG's dependency graph. Output of operation 1 is required in a delayed downstream consumer (op4) in addition to the adjacent consumer (op2). %The intermediate matrix cannot be overwritten or discarded, since its required in a future computation. 


%This complex dependency graph can often complicate the optimization of loop orders and tiling strategies to determine efficient intra-operation and inter-operation dataflows.


(2) CG has some tensor operations with contracted rank being much larger than the other ranks. This diminishes the benefit of pipelining because significant computation is required to produce any given final sum; therefore, making it a rate limiting step. 
%This prevents pipelining the entire graph.
%\TK{the following line seems out of place - since its one of many techniques we propose. Should maybe remove it}
%We propose \textit{pipelining with writeback}, which involves traditional pipelining and writing back the intermediate data to the buffer, hence incurring only write accesses and avoiding the read accesses for the intermediate matrix.

\insertFigure{no-fusion}{A part of the CG tensor dependency graph where a node represents the equation in~\autoref{alg:cg_einsum} and edge represents the output of the source node equation. The data cannot be consumed and be shielded from memory hierarchy since its reused again in another tensor. Please refer to ~\autoref{fig:dfg} for complete graph of CG.\vspace{-3mm}}%\RG{contraction heavy}}

(3) As the DAG becomes more complex, it is important to make sure that the loop order choice minimizes the data layout transformation (we use the term swizzling for it) of these tensors across various consumer operations.

(4) The downstream consumers also result in multiple \textit{tensor operand reuse distances}.

In this work, we identify various \textit{inter-operation} reuse opportunities to enhance the arithmetic intensity of such applications.
Our proposed \emph{generalized inter-operation reuse} is a wider generalization of \emph{traditional inter-operation pipelining}. We propose \DataflowName (\TitleExpansion), a strategy for mapping DAG of tensor operations which exploits reuse opportunities between operations.

\DataflowName is applicable to any DAG of operations. So while it helps extract reuse in the complex DAGs like CG, these patterns can also apply to simpler DAGs like GCNs, thus preserving generalizability.

%\reviewme{\DataflowName consists of the following contributions.

 %First, we identify the inter-operation reuse patterns in an arbitrary DAG of tensor operations. We propose a methodology to mark the edge of the DAG with the appropriate reuse pattern. This addresses the DAG complexity problems.

% Second, we propose loop orders that try to take the maximum advantage of the reuse patterns, given that the ability to extract reuse also depends upon the order of loops in these operations. The loop order also minimize swizzling

 %Third, prior works on pipelining~\cite{flat,tangram,garg2021understanding,yan2020hygcn}, divide the whole compute region into contiguous chunks and an operation is mapped on to a chunk as in~\autoref{fig:spacetime} (top sub-figure) shows. However, there is not much reuse within a single operation and the whole tensor needs to be communicated between the chunks. Instead, we pipeline within the cluster and split dominant ranks across cluster (\autoref{fig:spacetime} bottom).


% Fourth, given that we minimize swizzling, we propose a buffer management scheme that writes the data into the SRAM in the same order and skips the SRAM once its full. Then it reads the portion that's already in the SRAM first. We show that this can improve the op-by-op baseline considerably. We also propose buffer management strategies to prioritize operations with low reuse distances and high reuse frequencies.

% }

%In this work, we identify various \textit{inter-operation} reuse opportunities which are not limited to \textit{inter-operation pipelining}.
%Please note that \textit{inter-operation reuse} is a wider generalization of \textit{traditional inter-operation pipelining} here, since inter-operation pipelining only exploits reuse between consecutive operations. \autoref{fig:venn} shows the scope of our work on inter-operation dataflows compared to prior works on acceleration.
%One example is \textit{pipelining with writeback}

%Moreover, it is important to focus on leveraging the knowledge of future occurrence of the tensor beyond the immediate tensor. In CG, these tensor operands have variable \textit{tensor operand reuse distances}. This pattern is frequent in various scientific applications as~\autoref{sec:background} shows. This complex dependency graph can often complicate the determination of loop orders and tiling strategies to determine efficient intra-operation and inter-operation dataflows.

%Also, given that the graph of tensors becomes more complex, it is important to make sure that the loop order choice minimzes the transformation of layouts of these tensors across various operations where that tensor is used. We use the term \textit{swizzling} for the layout transformation. Thus we need to minimize swizzling.

%\RG{Can we cut this para and make contributions slightly longer ?}
%Based on the insights from the tensor dependency graphs of various applications, we propose a systematic methodology to identify, classify and exploit reuse opportunities in an arbitrary graph of tensor operations targeting spatial accelerators. This also involves deriving the loop orders and tile sizes for individual operations since the ability to exploit the inter-operation reuse can also depend on the individual operation's dataflow.
%Some other applications which have individual \GEMM of low arithmetic intensity include Graph Neural Network, Transformers etc. where our methodology is applicable, however, we often refer to Conjugate Gradient for demonstration purposes in this paper since its tensor dependency graph already has the characteristics of low intensity Graph and ML workloads but also has additional unique characteristics providing opportunity to demonstrate different kinds of inter-operation reuse.
%We also propose a scalable tiling strategy that involves splitting a memory bound GEMM by the dominating rank into sub-tensors and reusing the data in a fine-grained manner between the sub-tensors from different operations within a compute node as the bottom half of~\autoref{fig:spacetime} shows.
% (shown later in~\autoref{fig:spacetime})\TK{not sure if we need to cite a figure that'll come this late. Might be better to point to the section that will discuss this}. 
%
% We propose \DataflowName (\TitleExpansion), a strategy for mapping DAG of tensor operations which exploits reuse opportunities between operations. It comprises of identifying inter-operation reuse patterns from the DAG structure, loop-reordering and tiling based on those patterns and custom scratchpad management strategies. 
Our key contributions are as follows:
%\vspace{-5mm}

%\begin{itemize}
\squishlist
\item We characterize the challenge of skewed GEMMs/SpMMs in tensor-algebra applications and systematically formulate \emph{generalized inter-operation reuse opportunities} (beyond pipelining) in a DAG of operations (\autoref{sec:dataflows}).
%We also observe that these patterns are frequent across other HPC workloads which we discuss in ~\autoref{sec:background}.
%\item We propose a systematic methodology to formulate the data reuse opportunities in an arbitrary DAG of tensor operations and based on the reuse opportunities, we derive the loop orders and tile sizes.(\autoref{sec:dataflows}).
%\item We co-optimize the loop orders and tiling strategies for the GEMM operations in order to leverage reuse from both traditional inter-operation pipelining and distance based inter-operation reuse.
\item Based on the reuse opportunities, we derive loop orders for the operations that allow consumers to maximally reuse the data, and require minimum changes to memory layout~(\autoref{sec:loop}).
\item Prior works on pipelining~\cite{flat,tangram,garg2021understanding,yan2020hygcn} divide the whole compute region into contiguous chunks and an operation is mapped on to a chunk as~\autoref{fig:spacetime} (top sub-figure) shows. However, there is not much reuse within a single operation and the whole tensor needs to be communicated between the chunks. We propose a scalable inter-operation tiling strategy which splits the dominant rank across compute clusters and pipelines the operations within a cluster as~\autoref{fig:spacetime} (bottom) shows~(\autoref{sec:tiling}).  %a mapping that reduces memory accesses and communication at the tensor dependency graph level.
%\end{itemize}
\item We propose a buffer management scheme that writes the data into the SRAM in the same order and skips the SRAM once its full. Then it reads the portion that's already in the SRAM taking advantage of swizzle minimzation. We also propose buffer management strategies that prioritize operations with low reuse distances and high reuse frequencies~(\autoref{sec:tornado}). %the notion of Tensor-operand level reuse distance for such patterns and a tensor organization strategy inside the buffer hierarchy (\autoref{sec:tornado}).
\item \DataflowName achieves \reviewme {geomean 5.97x (ranging from 1.34x to 23x)} improvement in the arithmetic intensity over operation by operation execution~(\autoref{sec:eval}).

\item \reviewme{\DataflowName is generally applicable to diverse tensor applications as it applies to all DAG structures. We also evaluate it on GCNs and ResNets and obtain 2.71x and xx geomean improvement in arithemetic intensity over op-by-op baseline~(\autoref{sec:eval}).} 
%\item We propose a novel data orchestration technique \DataflowName which allows for efficient replacement, placement and prefetching of data for applications with variable reuse distance patterns. Since reuse distance is a generalization, \DataflowName can be used for applications with only intra-operation reuse and inter-operation pipelining opportunities as well.
%\item We propose a novel buffer idiom \TODO{name} which improves performance and energy over caches and scratchpads by \TODO{xx} and \TODO{xx}
\squishend
\end{comment}

\begin{comment}

\begin{enumerate}
    \item Identifying inter-operation reuse patterns in an arbitrary DAG of operations
    \item Deriving loop orders to make sure that they are amenable to inter-operation reuse and minimize swizzling
    \item Proposing tiling strategy that does pipelining within the compute node and splits the large rank across nodes (bottom half of~\autoref{fig:spacetime}).
    \item Proposing scratchpad management strategies like reuse distance and frequency based tensor replacement and proposing strategies to extract reuse from the portion of the tensor that does fit in SRAM.
    
\end{enumerate}
\vspace{-1mm}
Our methodology is also applicable to %(and evaluated on) 
other applications with low intensity GEMMs like GNNs and transformers. %where our methodology is applicable,
However, we often refer to Conjugate Gradient as the application for demonstration purposes since its tensor dependency graph has the characteristics of low intensity Graph and ML workloads and also has additional unique characteristics providing opportunity to demonstrate different kinds of inter-operation reuse.
\autoref{fig:venn} shows the scope of our work on inter-operation dataflows compared to prior works on accelerator dataflow.
%Our proposed \textit{inter-operation reuse} is a wider generalization of \textit{traditional inter-operation pipelining} here, since inter-operation pipelining only exploits reuse between consecutive operations.
%\autoref{fig:venn} shows the scope of our work on inter-operation dataflows compared to prior works on acceleration.

%Therefore data orchestration which accounts for such reuse is critical for HPC workloads. Cache replacement policies often have a global view of an individual line rather than a tensor as a whole, which limits the applicability for such algorithms. Moreover, LRU replacement does not see the future reuse of the tensor and replaces it if it has not been used recently. Belady's optimal replacement policy requires knowledge of future accesses for each line and often requires additional structures and meta data accesses to replace one line which is costly to implement~\cite{popt-hpca21}. Scratchpads, on the other hand provide ability to the programmer to have control over data orchestration. However, these scratchpads are often over-provisioned for the worst case applications.

%To this end, we propose \DataflowName data orchestration that analyzes the tensor operand-level reuse patterns in the algorithm and the dataflows of the individual GEMMs to manage the data in the memory hierarchy. \DataflowName also enables efficient prefetching for these HPC algorithms due to the knowledge of the future tensor reuse pattern and dataflows.

 %Some other applications with low arithmetic intensity include Graph Neural Network, Transformers etc., however, we often refer to Conjugate Gradient for demonstration purposes in this paper since its DAG already has the characteristics of Graph and ML workloads but also has additional unique characteristics providing opportunity to demonstrate different kinds of inter-operation reuse.


\noindent  \textbf{\textit{The key contributions of this paper are:}}
\end{comment}

%Our methodology is also applicable to %(and evaluated on) 
%other applications with low intensity GEMMs like GNNs and transformers. %where our methodology is applicable,
%However, we often refer to Conjugate Gradient as the application for demonstration purposes since its tensor dependency graph has the characteristics of low intensity Graph and ML workloads and also has additional unique characteristics providing opportunity to demonstrate different kinds of inter-operation reuse.
%\autoref{fig:venn} shows the scope of our work on inter-operation dataflows compared to prior works on accelerator dataflow.
%Our proposed \textit{inter-operation reuse} is a wider generalization of \textit{traditional inter-operation pipelining} here, since inter-operation pipelining only exploits reuse between consecutive operations.
%\autoref{fig:venn} shows the scope of our work on inter-operation dataflows compared to prior works on acceleration.


































\begin{comment}
\section{Problem and Motivation}
\label{sec:introduction}

Sparse and Dense matrix multiplications are prime operations for a variety of applications spanning Graph Analytics~\cite{kipf2017semisupervised,hamilton2017inductive}, High-Performance Computing~\cite{cools2017communication,cerebras} and Artificial Intelligence~\cite{resnet,nlp}. The GEMM operations used in DNNs offer vast reuse opportunities~\cite{kwon2019understanding,interstellar,timeloop,eyeriss2016isca} owing to their high arithmetic intensity. This has led to a plethora of spatial accelerators for DNN applications~\cite{eyeriss2016isca,kwon2018maeri,tpu-isca,nvdla,shi}. Prior works have also looked at the acceleration for Sparse workloads~\cite{sigma,eie,extensor,eyeriss2} by eliminating redundant matrix multiplications and memory accesses.

However, certain PDE solver algorithms used scientific applications like the Conjugate Gradient~\cite{hestenes1952methods} have SpMM/SpMV and GEMM/GEMV operations with low arithmetic intensity~\cite{cerebras}. The best supercomputers ranked on High-Performance Linpack benchmark are able to achieve only upto 3\% of the performance on the HPCG benchmark~\cite{cerebras,osti_1089988}.
~\autoref{alg:cg_einsum} shows the Block Conjugate Gradient Algorithm. ~\autoref{fig:results}a) and b) show maximum achievable arithmetic intensity of individual operations. Please note that instead of counting multiplications and additions separately, we count MAC as a unit of computation. We also consider matrix addition of, for example, $X^{k-1}$ with $P^{k-1}.\alpha^{k-1}$ in the equation $X^{k}=X^{k-1}+P^{k-1}\alpha^{k-1}$ to be done immediately after the MAC and we absorb the addition in same operation. Therefore, effectively we count number of multiplications per memory access of an element (independent of the bit precision). Please note, here number of RHS is a parameter with values 1,8,16,32 and 64. 

\insertFigure{cg}{Block CG Algorithm.}


~\autoref{fig:results}a) shows the maximum achievable arithmetic intensity for individual SpMM operations for the suitesparse CG matrices. We note that the SpMMs, especially the highly sparse ones like barth4 have extremely low arithmetic intensity even for RHS=64.
~\autoref{fig:results}b) shows the maximum achievable arithmetic intensity of dense GEMMs in an individual operation in terms of number of multiplications per memory access. We notice that the arithmetic intensity of the DenseGEMMs is severely limited by the number of RHS (ie. the number of problems solved simultaneously.) Therefore traditional DNN accelerators~\cite{eyeriss2016isca,kwon2018maeri,tpu-isca} do not help accelerate these workloads due to fundamentally low reuse.

~\autoref{fig:results}c) shows the arithmetic intensity for one iteration of the CG loop. Please note that for matrix inverse, we consider LU factorization followed by Triangular Solve. Also, we conservatively count accesses to $P$ and $P^T$ separately owing to different layout in the memory. We note that the amount of reuse that can be extracted between the operations is high and this motivates us to design a new dataflow for HPCG workloads which tries to maximize inter-operation rather than optimizing for inter-operation reuse.

\end{comment}

==> 01-Introduction.tex <==
%\vspace{-3mm}
\section{Introduction}
\label{sec:introduction}


\begin{comment}
    Points to be made in the intro
        - High value GEMM workloads have complex dependencies []
        - Traditional pipelining does not respond well to these dependencies
        -Keeping operands on-chip is key to get a good performance.
                - Caches - Implicit and Workload agnostic + hardware overheads
                - Spads - Explicitly managed (large map-space and expensive search and buffer allocation)
                - CHORD: A hybrid implicit and explicit management, which is cycle-level implicit and coarse-grained explicit, so the cost lowers enough to manage the SRAM online..
        - SCORE: Fast scheduler for low intensity ops that deals with more complex dependencies, and also provides metadata to CHORD..
        - Skewed GEMMs can have surprisingly low arithmetic intensity??
        
    


    
\end{comment}





As Deep Learning (DL) emerged as a high-value workload, the computer architecture community responded by proposing custom accelerators for DNNs~\cite{eyeriss2016isca,kwon2018maeri,tpu-isca,nvdla}. 
The most common fundamental operation for these DNNs was matrix multiplication, often expanded from convolutional layers that were common in DNNs at that time. These GEMMs offered good reuse opportunities because of their large dimensions and relatively cubic aspect ratios, allowing early DNN accelerators to successfully schedule each layer independently and achieve maximum utilization for the networks they targeted at design-time. Simultaneously, these schedules could be efficiently implemented using \emph{scratchpad} buffers that were explicitly controlled by the schedule to the stage intermediate \emph{tiles} of data according to the traversal order within each GEMM, without concern for inter-layer efficiency.

%Furthermore, prior works have also looked at the accelerators for sparse tensor workloads~\cite{sigma,eie,extensor,eyeriss2} which eliminate irrelevant multiplications and memory accesses.}% Unfortunately, this approach lowers intensity even further, and straightforwardly applying these to CG on a GEMM-by-GEMM operation basis results in compute under-utilization due to limited memory bandwidth.


Recently, work like the Tensor Algebra COmplier (TACO) \cite{XXXTaco} has spurred research interest in generalized tensor applications, including sparse tensor algebra. %The computer architecture community has responded with recent proposals that generalize custom accelerators to efficiently target a superset of DNNs \cite{extensor, tensaurus, dave2020hardware, tensorlib, flextensor} namely, applications represented as arbitrary DAGs of \emph{tensor operations} and non-linearities for DL activation functions.
However, this generalization brings new challenges: tensor-algebra applications have diverse shapes, sparsity ratios, and dependency graphs. %Worse, this is coupled with a trend in DNNs away from large, monolithic GEMMs and towards numerous small independent matrix multiplications\footnote{Often called \emph{batched} GEMMs, which should not be confused with DNN batch size.} with less cubic aspect ratios.
This is significant because of an underappreciated fundamental property: namely, \textit{not all dense GEMMs with large number of multiplications are compute-bound even in the best case}. As shown in \autoref{fig:ai1}, a \emph{skewed} aspect ratio inherently decreases \emph{arithmetic intensity} (AI), thus making the individual GEMM memory-bound and leaving datapath resources idle. For example, to saturate its datapaths the TPU v3 and v4 architectures require an AI of approximately 150 and 250 respectively~\cite{tpuv4}.  %Sparse tensor algebra introduces similar challenges, as removing multiplication-by-zero decreases the AI numerator, while transferring \emph{metadata} for compression formats increases the denominator relatively.}

\insertFigureScaled{ai1}{Degradation of arithmetic intensity on two GEMMs with the same number of multiplications due to aspect ratio skew.\vspace{-3mm}}{.75}



%\insertFigure{no-fusion}{Pipelining cannot simply be applied to complex DAGs due to - 1) Delayed downstream dependency, 2) varying shapes, 3) consumers at multiple reuse distances 4) need to preserve layout across conusmers.\vspace{-3mm}}


%The reason for this is low arithmetic intensity for a skewed GEMM and it can be as low below 1 op/byte. Currently, most scheduling strategies optimize matrix multiplications independently and compose them to execute in an op-by-op manner, which leads to low performance in applications with skewed GEMMs.}

\begin{comment}
A real-world quantification of this phenomenon is captured by HPCG benchmark~\cite{dongarra2015hpcg,hpcg2021}, which runs Conjugate Gradient (CG)---a widely used HPC solver application represented as a DAG of tensor operations.

\input{tables/hpcg}

%\footnote{HPCG is a benchmark for supercomputers that runs CG. \MP{Footnote 1 adds no real information. Cut. }}
As \autoref{tables:hpcg} shows, CG achieves only 1-3\% of peak performance on top 7 supercomputers. 
Therefore, intra-operation reuse alone is not sufficient.
The overall throughput can be increased by improving the arithmetic intensity (i.e., on-chip data reuse), which can be done by seeking inter-operation reuse.
\end{comment}

Thus to achieve full utilization we must consider inter-GEMM operation scheduling. Prior works have also shown that simple pipelining of adjacent operation~\cite{tileflow,isca-pip,yan2020hygcn} can improve things, but these solutions exclude significant potential sources of reuse, including delayed downstream consumers, and multiple consumers with varying reuse distances or traversal orders as~\autoref{fig:no-fusion} shows. To make matters worse, these extra options explode the scheduling space for finding good scratchpad configurations, as the total combinations and proportions of allocations explodes with operation DAG depth and the number of tensors involved. This means that exhaustive schedule-space exploration techniques become unacceptably slow, and also that heuristic solutions are more likely to miss the true optimal.

%It is also challenging to simply apply traditional inter-operation pipelining in cases of these dependencies, because of the delayed downstream dependencies, varying shapes of skewed GEMMs and multiple of these downstream consumers as~\autoref{fig:no-fusion} shows. %\TK{Fig 4 getting referenced before Fig 3, i suggest bring it before Fig 4 then} 
%~\autoref{fig:dfg} shows an actual complex cascade of tensor operations found in CG, a high-value HPC workload rich in these complexities.
%Thus, we need mechanisms to cache these intermediate tensors within SRAMs, since there are situations where simple pipelining cannot be applied.

%Prior works like buffets~\cite{buffets} make use of \emph{explicit decoupled data orchectration} to supplement scratchpad RAM with simple pointer and credit management scoreboarding. This is called explicit because data placement and RAM replacement are schedule-controlled, and decoupled because it operates on bulk-synchronous fills. %These work well for executing one layer at a time, when all dimensions of matrices have sufficient reuse.
%While explicit orchestration works well for scheduling single matrix multiplication at a time, considering data placement, for inter-operation reuse statically in general tensor algebra is a diabolically hard problem. 
% In order to reuse such operands, specially where intra-operation reuse is simply not enough, storing these operands in the on-chip buffer is essential, and multiple of these operands contend for space inside the buffer. We show in~\autoref{sec:arguments} that the design-space to accommodate multiple tensors inside a buffer space explodes in complexity. ~\autoref{sec:arguments} also discusses why running statically known DAGs does not necessarily imply that scratchpads are not burdensome and don't have design-time overheads.
%Overall, the co-dependence on schedule, available scratchpad capacity and different downstream consumers make the explicit scheduling problem too challenging.

\insertFigure{no-fusion}{Pipelining cannot simply be applied to complex DAGs due to - 1) Delayed downstream dependency, 2) varying shapes, 3) consumers at multiple reuse distances 4) need to preserve layout across conusmers. We discuss this in detail in~\autoref{sec:nofusion}\vspace{-3mm}}

Of course, scratchpads can be supplemented with pointer and credit management logic to become queues or buffets~\cite{buffets}, but these do not solve the schedule explosion problem as their staging decisions are still \emph{explicitly} controlled. Alternatively, caches are widespread on-chip storage structures that use \emph{implicit} data orchestration. Ideally, the presence of the cache is not architecturally exposed and the hardware itself does the best job possible of reusing the data. (In practice, best optimization is often made by cache-aware scheduling policies, blurring the line between implicit and explicit.) However, the area and energy overhead for tag matching make it less appealing for custom accelerators, as well as the possibility of increased misses due to conflicts. Overheads aside, cache policies typically operate at line granularity of unified address streams, rather than having higher-level knowledge of tensors, blocks, or intended reuse distance. This results in cache policies often rejecting the data that may have high reuse frequency (by virtue of reuse of the whole block) but might not be the immediate vicinity (i.e., high reuse distance).

In order to effectively exploit all available sources of reuse, we propose a unique approach: co-designing the buffer storage idiom with the scheduling algorithm. Our goal is that it becomes tractable to find schedules that obtain a sufficient level of inter-operation reuse to reach the compute bound, even in the face of complex DAGs of dependencies. To achieve this, we propose ~\SpadNamenospace\footnote{\SpadNameexp}, a novel \emph{explicit+implicit hybrid} buffering scheme that aims to combine the ``best of both worlds'' by placing coarse-grained decisions under the explicit control of the scheduler for efficiency, while making low-level fine-grained decisions implicitly like a cache, thus significantly reducing the size of the schedule space.
%~\SpadName is workload-aware, as it uses high-level metadata like starting and ending global address of a tensor, tensor-level reuse frequency and distance from the workload (the explicit component), but implicitly controls placement of elements of tensors without being burdensome to the programmer. ~%\TK{it might be worth adding a footnote saying you use scratchpad and buffer interchangeably in this paper} 
%\TK{based on what the footnote says its unclear whether chord is a scratchpad or cache }
Notably, this approach also significantly reduces the area and energy overheads of traditional line-level caches. %Specifically,~\SpadName uses per-tensor replacement policies that can be configured by the schedule at coarse granularity.
%for operands with downstream consumers that uses implicit replacement at a tensor granularity rather than a line granularity. 
%In this work we propose two such policies- \\(1) \PolicyA - \SpadName is filled in the queue order and once the buffer is full, the spilling data is sent straight to the DRAM.\\
%(2) \PolicyBnospace\footnote{\PolicyBexp} - If the current tensor has a higher reuse frequency and lower reuse distance (in case of same frequency) than the previously written tensor, the current tensor starts replacing the previous tensor by the tail.
%Because of its extremely coarsened granularity, ~\SpadName retains the benefit of a scratchpad over a cache (i.e., with minimal (<1\% of that of cache) tag matching overhead) 
%Hence it gets rid of caches' tag matching overhead and 
%while
%our proposed implicit tensor replacement policies~\PolicyA and \PolicyB remove the challenge of statically coming up with the data placement and replacement strategies statically for operands in multiple operations.

To schedule accelerators that use this structure, we propose ~\DataflowNamenospace\footnote{\DataflowNameexp} a downstream dependency aware novel scheduling strategy. 
\DataflowName identifies the delayed downstream dependencies that require writeback from those where pipelining would work, and steers the tensors with delayed writeback dependencies to~\SpadNamenospace. In order to exploit the reuse on delayed downstream consumers, it is important to make sure that the order in which the elements are produced as same as the order in which they are consumed, otherwise, layout transformation is required. Unlike prior mappers which search for tile-sizes for fine-grained buffer allocation, \DataflowNamenospace's involvement in buffer allocation is coarse-grained at an operand granularity rather than element-wise granularity, and low-level fine-grained decisions are made implicitly by~\SpadNamenospace's policies. 

All in all, we show that \SpadName and \DataflowName are applicable to diverse tensor applications and achieve 2.51x geomean speedup and 4x improvement in energy efficiency across a broad range of workloads (\autoref{sec:eval}).

%\TK{minimizing layout transformation is an important feature. Lets highlight it more explcitly. As in mention that the dataflow of the current op and downstream op may be different requiring expensive layout transformation, and SCORE tries to minimize that.}%It consists of the following steps - \\ 
%\TK{there seems to be some missing text here?}
%(1) Marking all the edges in the DAG of tensor operations with pipelining opportunities. This is useful in situations where tensors have delayed downstream consumers which can be visualized as a long edge in the DAG.\\
%(2) Assigning loop orders and tiling strategies to ensure that pipelining is actually exploited and layout transformation overhead of a tensor is minimized.\\
%\DataflowName reduces the contending tensors and also ensures minimum layout transformation (aka swizzling) which is also the motivation behind~\PolicyA policy.
%The main reason is the low arithmetic intensity achieved by the execution of Conjugate Gradient on CPUs/GPUs. 
%The main reason for this that the tensor multiplications---which we term \emph{operation} for this paper---%\MP{This definition is also too important to be in a footnote
 %used in CG have extremely unbalanced aspect ratios, which significantly lowers arithmetic intensity and data reuse.} %\MP{I feel like this point should come earlier, perhaps before the previous paragraph.}
%We use the term \emph{skewed} GEMMs to refer to such SpMMs/GEMMs---though notably, in the limit they can devolve to matrix-vector multiplication, i.e. if the shape of the matrix is 100,000:8.}%The main reason for this is costly data movement and communication between compute clusters/pods\MP{This explanation doesn't make sense either. Needs a reuse/intensity component. Even if this made sense, does GOGETA actually fix this problem?}.




%\TK{@Raveesh - I think we can move this para to para 3. Basically start with current para 2 on GEMMs, reuse and spatial accelerators. Then introduce CG. So intersperse this para with current para 3}


%making inter-operation reuse essential.

%This work explores inter-operation reuse opportunities for kernels like CG to enhance its arithmetic intensity.

%However, the~\GEMM in CG have orders of magnitude lower arithmetic intensity compared to SpMMs/GEMMs in DNNs and offer less reuse opportunities within one operation as~\autoref{fig:ai}~(\autoref{sec:ai}) discusses later in the paper. 
%Thus, executing CG at the granularity of a GEMM, reading tensors from DRAM and writing the output of each GEMM to DRAM, makes it highly memory bound leading to low compute utilization as~\autoref{\:hpcg} shows. 
\begin{comment}
Fusing \textit{adjacent} low AI matrix multiplication operators has recently been leveraged for applications like Graph Convolutional Networks (GCN)~\cite{garg2021understanding,yan2020hygcn,liang2020engn} and Transformers~\cite{flat,flashattention} 
wherein tiles of the intermediate tensor are manifested and consumed within the 
on-chip memory hierarchy in a \textit{pipelined} manner, reducing  intermediate output data movement to and from DRAM. We call this \emph{adjacent-op pipelining} in this work.
Other recent works have looked at enumerating the design-space for such adjacent-op pipelining~\cite{garg2021understanding} and 
%\TK{is this what the isca paper does?}\RG{Yep}
identifying optimal pipelined dataflow choices~\cite{isca-pip}, thereby enhancing better compute utilization when running memory-bound tensors.

While traditional adjacent-op pipelining is promising for DAGs with linear chains of operators (i.e., most DNNs today and GCNs), we show in this work that it is insufficient to capture nuances in more complex DAGs, such as those used in HPC kernels like CG.
Specifically, delayed downstream consumption of fanout of tensors, implies that traditional pipelining which overwrites the previously consumed tile cannot be applied directly due to a later dependency.%~\autoref{fig:no-fusion} shows an example, where tensor S has a delayed consumer.
 Moreover nuances such as data layouts of one tensor consumed in various operations is not captured by adjacent pipelining.
%that prior works cannot capture, as we discuss later. \autoref{table:related} enumerates this.

In this work, we coin the term \emph{generalized inter-operation reuse} to widen the scope of inter-operation reuse beyond adjacent operators to include additional reuse opportunities (\autoref{table:related}).
%as a wider generalization of traditional \emph{adjacent-operator pipelining}, introducing three additional reuse opportunities (\autoref{table:related}). 
We also propose \DataflowName (\TitleExpansion), which is a systematic strategy for mapping DAG of tensor operations exploiting the generalized inter-operation reuse opportunities, with the goal of enhancing the AI of the overall application.
%\DataflowName is applicable to any DAG of operations. 
We demonstrate that while \DataflowName is essential for extracting reuse in complex DAGs like CG, it can also be applied to simpler DAGs like GCNs and DNNs, thus preserving generalizability.

%\insertFigurePartnnnn{no-fusion}{A part of the CG tensor dependency graph where a node represents the equation in~\autoref{alg:cg_einsum} and edge represents the output of the source node equation. Please refer to ~\autoref{fig:dfg} for complete graph of CG.\vspace{-3mm}}%\RG{contraction heavy}}
We summarize our contributions below:
%\TK{I think the contribitions can be listed more succinctly. I would suggest each contribution bullet pointing to a specific section of paper. }

\squishlist
%\item We characterize the challenge of skewed GEMMs/SpMMs in tensor-algebra applications and the challenges of generalizing traditional inter-operation pipelining~\footnote{Not to be confused with inter-operation "reuse" since pipelining is a narrow aspect of inter-operation reuse}. (\autoref{sec:ai}).
%We also observe that these patterns are frequent across other HPC workloads which we discuss in ~\autoref{sec:background}.
%\item We propose a systematic methodology to formulate the data reuse opportunities in an arbitrary DAG of tensor operations and based on the reuse opportunities, we derive the loop orders and tile sizes.(\autoref{sec:dataflows}).
%\item We co-optimize the loop orders and tiling strategies for the GEMM operations in order to leverage reuse from both traditional inter-operation pipelining and distance based inter-operation reuse.

\item We propose~\DataflowName (\autoref{sec:score}), a scheduler which identifies the operands with delayed dependencies that require writeback (and hence \SpadNamenospace), and proposes a schedule that maximizes inter-operation reuse and minimizes the layout transformation of the operands across different consumers.
\item We propose~\SpadName(\autoref{sec:chorus}), a buffer structure for operands with downstream consumers that uses tensor-operand level replacement, that reduces tag match overhead and considers a more wholistic view of the object rather than a cache line. Cycle-level implicit tensor level replacement also eases the burden of solving tensor allocation involving multiple tensors statically which is a hard problem. 
%\item %Prior works on pipelining~\cite{flat,tangram,garg2021understanding,yan2020hygcn} divide the whole compute region into contiguous chunks and an operation is mapped on to a chunk as~\autoref{fig:spacetime} (top sub-figure) shows.\TK{seems odd to cite Fig 12 in intro}
%However, there is not much reuse within a single operation and the whole tensor needs to be communicated between the chunks. 
%\TK{this seems like a very specific optimization - and confusing here about what is lower BW vs higher BW NoC .. in fact i dont recall our arch section / Table IV talking about two NoCs with diff BWs? cant you state this contribution more generally about a communication BW optimized scalable inter-operation tiling strategy?}
%We propose a scalable inter-operation tiling strategy that reduces inter-cluster communication(~\autoref{sec:tiling}).  %a mapping that reduces memory accesses and communication at the tensor dependency graph level.
%\end{itemize}
%\item We propose buffer management schemes that reuse initial tiles of the output and can also replace the tensor based on future reuse distance and frequency~(\autoref{sec:tornado}). %the notion of Tensor-operand level reuse distance for such patterns and a tensor organization strategy inside the buffer hierarchy (\autoref{sec:tornado}).

\item We demonstrate the limitations of caches, namely, area overhead and line-level policies and the limitations of scratchpad, namely complexities in static buffer allocation of multiple delayed downstream consumers (\autoref{sec:arguments}).

\item We show that \SpadName and \DataflowName are applicable to diverse tensor applications and achieve 2.51x geomean speedup and 4x improvement in energy efficiency across a broad range of workloads (\autoref{sec:eval}).

%\item \reviewme{ } 
%\item We propose a novel data orchestration technique \DataflowName which allows for efficient replacement, placement and prefetching of data for applications with variable reuse distance patterns. Since reuse distance is a generalization, \DataflowName can be used for applications with only intra-operation reuse and inter-operation pipelining opportunities as well.
%\item We propose a novel buffer idiom \TODO{name} which improves performance and energy over caches and scratchpads by \TODO{xx} and \TODO{xx}
\squishend
\end{comment}


\begin{comment}
\emph{Inter-operation pipelining (aka fusion)} has been shown to be beneficial for accelerators for applications like Graph Neural Networks~\cite{garg2021understanding,yan2020hygcn,liang2020engn} where the intermediate tensor is reused between an SpMM and a GEMM,  reducing  intermediate output data movement to and from DRAM.
It has been shown that this approach is more challenging~\cite{dnnfusion,flat} and has a larger design-space~\cite{garg2021understanding} than straightforward element-wise fusion done by ML compilers today, for example, matrix-multiplication and ReLU fusion.
%Unfortunately, \textit{traditional inter-operation pipelining} often consumes the intermediate data and does not keep it in the memory. 
%Traditionally, \textit{inter-operation pipelining} has been exploited in prior works~\cite{tangram,garg2021understanding,yan2020hygcn,flat} %across various application domains 
%to reduce the data movement to DRAM, by consuming the portion of the tensor as it is produced 
\TK{I think we need to transition to saying that inter-operation pipelining does not capture all inter-operation reuse opportunities as this work identifies.}
Unfortunately, the additional complexity of inter-operation dependency graphs in certain applications introduces additional challenges which confounds the attempts at \emph{traditional inter-operation pipelining.} Furthermore, just capturing reuse in adjacent operations misses the overall opportunity to consider future instances of reuse of tensors in the entire program. \reviewme{We use CG as an example to discuss these challenges and missed opportunities:}

(1) Operations can have a delayed downstream consumer. Therefore, the data must remain resident in the memory hierarchy. However, traditional pipelining overwrites tiles that are consumed by the adjacent operation.
%~\autoref{fig:dfg} shows CG's dependency graph. Output of operation 1 is required in a delayed downstream consumer (op4) in addition to the adjacent consumer (op2). %The intermediate matrix cannot be overwritten or discarded, since its required in a future computation. 


%This complex dependency graph can often complicate the optimization of loop orders and tiling strategies to determine efficient intra-operation and inter-operation dataflows.


(2) CG has some tensor operations with contracted rank being much larger than the other ranks. This diminishes the benefit of pipelining because significant computation is required to produce any given final sum; therefore, making it a rate limiting step. 
%This prevents pipelining the entire graph.
%\TK{the following line seems out of place - since its one of many techniques we propose. Should maybe remove it}
%We propose \textit{pipelining with writeback}, which involves traditional pipelining and writing back the intermediate data to the buffer, hence incurring only write accesses and avoiding the read accesses for the intermediate matrix.

\insertFigure{no-fusion}{A part of the CG tensor dependency graph where a node represents the equation in~\autoref{alg:cg_einsum} and edge represents the output of the source node equation. The data cannot be consumed and be shielded from memory hierarchy since its reused again in another tensor. Please refer to ~\autoref{fig:dfg} for complete graph of CG.\vspace{-3mm}}%\RG{contraction heavy}}

(3) As the DAG becomes more complex, it is important to make sure that the loop order choice minimizes the data layout transformation (we use the term swizzling for it) of these tensors across various consumer operations.

(4) The downstream consumers also result in multiple \textit{tensor operand reuse distances}.

In this work, we identify various \textit{inter-operation} reuse opportunities to enhance the arithmetic intensity of such applications.
Our proposed \emph{generalized inter-operation reuse} is a wider generalization of \emph{traditional inter-operation pipelining}. We propose \DataflowName (\TitleExpansion), a strategy for mapping DAG of tensor operations which exploits reuse opportunities between operations.

\DataflowName is applicable to any DAG of operations. So while it helps extract reuse in the complex DAGs like CG, these patterns can also apply to simpler DAGs like GCNs, thus preserving generalizability.

%\reviewme{\DataflowName consists of the following contributions.

 %First, we identify the inter-operation reuse patterns in an arbitrary DAG of tensor operations. We propose a methodology to mark the edge of the DAG with the appropriate reuse pattern. This addresses the DAG complexity problems.

% Second, we propose loop orders that try to take the maximum advantage of the reuse patterns, given that the ability to extract reuse also depends upon the order of loops in these operations. The loop order also minimize swizzling

 %Third, prior works on pipelining~\cite{flat,tangram,garg2021understanding,yan2020hygcn}, divide the whole compute region into contiguous chunks and an operation is mapped on to a chunk as in~\autoref{fig:spacetime} (top sub-figure) shows. However, there is not much reuse within a single operation and the whole tensor needs to be communicated between the chunks. Instead, we pipeline within the cluster and split dominant ranks across cluster (\autoref{fig:spacetime} bottom).


% Fourth, given that we minimize swizzling, we propose a buffer management scheme that writes the data into the SRAM in the same order and skips the SRAM once its full. Then it reads the portion that's already in the SRAM first. We show that this can improve the op-by-op baseline considerably. We also propose buffer management strategies to prioritize operations with low reuse distances and high reuse frequencies.

% }

%In this work, we identify various \textit{inter-operation} reuse opportunities which are not limited to \textit{inter-operation pipelining}.
%Please note that \textit{inter-operation reuse} is a wider generalization of \textit{traditional inter-operation pipelining} here, since inter-operation pipelining only exploits reuse between consecutive operations. \autoref{fig:venn} shows the scope of our work on inter-operation dataflows compared to prior works on acceleration.
%One example is \textit{pipelining with writeback}

%Moreover, it is important to focus on leveraging the knowledge of future occurrence of the tensor beyond the immediate tensor. In CG, these tensor operands have variable \textit{tensor operand reuse distances}. This pattern is frequent in various scientific applications as~\autoref{sec:background} shows. This complex dependency graph can often complicate the determination of loop orders and tiling strategies to determine efficient intra-operation and inter-operation dataflows.

%Also, given that the graph of tensors becomes more complex, it is important to make sure that the loop order choice minimzes the transformation of layouts of these tensors across various operations where that tensor is used. We use the term \textit{swizzling} for the layout transformation. Thus we need to minimize swizzling.

%\RG{Can we cut this para and make contributions slightly longer ?}
%Based on the insights from the tensor dependency graphs of various applications, we propose a systematic methodology to identify, classify and exploit reuse opportunities in an arbitrary graph of tensor operations targeting spatial accelerators. This also involves deriving the loop orders and tile sizes for individual operations since the ability to exploit the inter-operation reuse can also depend on the individual operation's dataflow.
%Some other applications which have individual \GEMM of low arithmetic intensity include Graph Neural Network, Transformers etc. where our methodology is applicable, however, we often refer to Conjugate Gradient for demonstration purposes in this paper since its tensor dependency graph already has the characteristics of low intensity Graph and ML workloads but also has additional unique characteristics providing opportunity to demonstrate different kinds of inter-operation reuse.
%We also propose a scalable tiling strategy that involves splitting a memory bound GEMM by the dominating rank into sub-tensors and reusing the data in a fine-grained manner between the sub-tensors from different operations within a compute node as the bottom half of~\autoref{fig:spacetime} shows.
% (shown later in~\autoref{fig:spacetime})\TK{not sure if we need to cite a figure that'll come this late. Might be better to point to the section that will discuss this}. 
%
% We propose \DataflowName (\TitleExpansion), a strategy for mapping DAG of tensor operations which exploits reuse opportunities between operations. It comprises of identifying inter-operation reuse patterns from the DAG structure, loop-reordering and tiling based on those patterns and custom scratchpad management strategies. 
Our key contributions are as follows:
%\vspace{-5mm}

%\begin{itemize}
\squishlist
\item We characterize the challenge of skewed GEMMs/SpMMs in tensor-algebra applications and systematically formulate \emph{generalized inter-operation reuse opportunities} (beyond pipelining) in a DAG of operations (\autoref{sec:dataflows}).
%We also observe that these patterns are frequent across other HPC workloads which we discuss in ~\autoref{sec:background}.
%\item We propose a systematic methodology to formulate the data reuse opportunities in an arbitrary DAG of tensor operations and based on the reuse opportunities, we derive the loop orders and tile sizes.(\autoref{sec:dataflows}).
%\item We co-optimize the loop orders and tiling strategies for the GEMM operations in order to leverage reuse from both traditional inter-operation pipelining and distance based inter-operation reuse.
\item Based on the reuse opportunities, we derive loop orders for the operations that allow consumers to maximally reuse the data, and require minimum changes to memory layout~(\autoref{sec:loop}).
\item Prior works on pipelining~\cite{flat,tangram,garg2021understanding,yan2020hygcn} divide the whole compute region into contiguous chunks and an operation is mapped on to a chunk as~\autoref{fig:spacetime} (top sub-figure) shows. However, there is not much reuse within a single operation and the whole tensor needs to be communicated between the chunks. We propose a scalable inter-operation tiling strategy which splits the dominant rank across compute clusters and pipelines the operations within a cluster as~\autoref{fig:spacetime} (bottom) shows~(\autoref{sec:tiling}).  %a mapping that reduces memory accesses and communication at the tensor dependency graph level.
%\end{itemize}
\item We propose a buffer management scheme that writes the data into the SRAM in the same order and skips the SRAM once its full. Then it reads the portion that's already in the SRAM taking advantage of swizzle minimzation. We also propose buffer management strategies that prioritize operations with low reuse distances and high reuse frequencies~(\autoref{sec:tornado}). %the notion of Tensor-operand level reuse distance for such patterns and a tensor organization strategy inside the buffer hierarchy (\autoref{sec:tornado}).
\item \DataflowName achieves \reviewme {geomean 5.97x (ranging from 1.34x to 23x)} improvement in the arithmetic intensity over operation by operation execution~(\autoref{sec:eval}).

\item \reviewme{\DataflowName is generally applicable to diverse tensor applications as it applies to all DAG structures. We also evaluate it on GCNs and ResNets and obtain 2.71x and xx geomean improvement in arithemetic intensity over op-by-op baseline~(\autoref{sec:eval}).} 
%\item We propose a novel data orchestration technique \DataflowName which allows for efficient replacement, placement and prefetching of data for applications with variable reuse distance patterns. Since reuse distance is a generalization, \DataflowName can be used for applications with only intra-operation reuse and inter-operation pipelining opportunities as well.
%\item We propose a novel buffer idiom \TODO{name} which improves performance and energy over caches and scratchpads by \TODO{xx} and \TODO{xx}
\squishend
\end{comment}

\begin{comment}

\begin{enumerate}
    \item Identifying inter-operation reuse patterns in an arbitrary DAG of operations
    \item Deriving loop orders to make sure that they are amenable to inter-operation reuse and minimize swizzling
    \item Proposing tiling strategy that does pipelining within the compute node and splits the large rank across nodes (bottom half of~\autoref{fig:spacetime}).
    \item Proposing scratchpad management strategies like reuse distance and frequency based tensor replacement and proposing strategies to extract reuse from the portion of the tensor that does fit in SRAM.
    
\end{enumerate}
\vspace{-1mm}
Our methodology is also applicable to %(and evaluated on) 
other applications with low intensity GEMMs like GNNs and transformers. %where our methodology is applicable,
However, we often refer to Conjugate Gradient as the application for demonstration purposes since its tensor dependency graph has the characteristics of low intensity Graph and ML workloads and also has additional unique characteristics providing opportunity to demonstrate different kinds of inter-operation reuse.
\autoref{fig:venn} shows the scope of our work on inter-operation dataflows compared to prior works on accelerator dataflow.
%Our proposed \textit{inter-operation reuse} is a wider generalization of \textit{traditional inter-operation pipelining} here, since inter-operation pipelining only exploits reuse between consecutive operations.
%\autoref{fig:venn} shows the scope of our work on inter-operation dataflows compared to prior works on acceleration.

%Therefore data orchestration which accounts for such reuse is critical for HPC workloads. Cache replacement policies often have a global view of an individual line rather than a tensor as a whole, which limits the applicability for such algorithms. Moreover, LRU replacement does not see the future reuse of the tensor and replaces it if it has not been used recently. Belady's optimal replacement policy requires knowledge of future accesses for each line and often requires additional structures and meta data accesses to replace one line which is costly to implement~\cite{popt-hpca21}. Scratchpads, on the other hand provide ability to the programmer to have control over data orchestration. However, these scratchpads are often over-provisioned for the worst case applications.

%To this end, we propose \DataflowName data orchestration that analyzes the tensor operand-level reuse patterns in the algorithm and the dataflows of the individual GEMMs to manage the data in the memory hierarchy. \DataflowName also enables efficient prefetching for these HPC algorithms due to the knowledge of the future tensor reuse pattern and dataflows.

 %Some other applications with low arithmetic intensity include Graph Neural Network, Transformers etc., however, we often refer to Conjugate Gradient for demonstration purposes in this paper since its DAG already has the characteristics of Graph and ML workloads but also has additional unique characteristics providing opportunity to demonstrate different kinds of inter-operation reuse.


\noindent  \textbf{\textit{The key contributions of this paper are:}}
\end{comment}

%Our methodology is also applicable to %(and evaluated on) 
%other applications with low intensity GEMMs like GNNs and transformers. %where our methodology is applicable,
%However, we often refer to Conjugate Gradient as the application for demonstration purposes since its tensor dependency graph has the characteristics of low intensity Graph and ML workloads and also has additional unique characteristics providing opportunity to demonstrate different kinds of inter-operation reuse.
%\autoref{fig:venn} shows the scope of our work on inter-operation dataflows compared to prior works on accelerator dataflow.
%Our proposed \textit{inter-operation reuse} is a wider generalization of \textit{traditional inter-operation pipelining} here, since inter-operation pipelining only exploits reuse between consecutive operations.
%\autoref{fig:venn} shows the scope of our work on inter-operation dataflows compared to prior works on acceleration.


































\begin{comment}
\section{Problem and Motivation}
\label{sec:introduction}

Sparse and Dense matrix multiplications are prime operations for a variety of applications spanning Graph Analytics~\cite{kipf2017semisupervised,hamilton2017inductive}, High-Performance Computing~\cite{cools2017communication,cerebras} and Artificial Intelligence~\cite{resnet,nlp}. The GEMM operations used in DNNs offer vast reuse opportunities~\cite{kwon2019understanding,interstellar,timeloop,eyeriss2016isca} owing to their high arithmetic intensity. This has led to a plethora of spatial accelerators for DNN applications~\cite{eyeriss2016isca,kwon2018maeri,tpu-isca,nvdla,shi}. Prior works have also looked at the acceleration for Sparse workloads~\cite{sigma,eie,extensor,eyeriss2} by eliminating redundant matrix multiplications and memory accesses.

However, certain PDE solver algorithms used scientific applications like the Conjugate Gradient~\cite{hestenes1952methods} have SpMM/SpMV and GEMM/GEMV operations with low arithmetic intensity~\cite{cerebras}. The best supercomputers ranked on High-Performance Linpack benchmark are able to achieve only upto 3\% of the performance on the HPCG benchmark~\cite{cerebras,osti_1089988}.
~\autoref{alg:cg_einsum} shows the Block Conjugate Gradient Algorithm. ~\autoref{fig:results}a) and b) show maximum achievable arithmetic intensity of individual operations. Please note that instead of counting multiplications and additions separately, we count MAC as a unit of computation. We also consider matrix addition of, for example, $X^{k-1}$ with $P^{k-1}.\alpha^{k-1}$ in the equation $X^{k}=X^{k-1}+P^{k-1}\alpha^{k-1}$ to be done immediately after the MAC and we absorb the addition in same operation. Therefore, effectively we count number of multiplications per memory access of an element (independent of the bit precision). Please note, here number of RHS is a parameter with values 1,8,16,32 and 64. 

\insertFigure{cg}{Block CG Algorithm.}


~\autoref{fig:results}a) shows the maximum achievable arithmetic intensity for individual SpMM operations for the suitesparse CG matrices. We note that the SpMMs, especially the highly sparse ones like barth4 have extremely low arithmetic intensity even for RHS=64.
~\autoref{fig:results}b) shows the maximum achievable arithmetic intensity of dense GEMMs in an individual operation in terms of number of multiplications per memory access. We notice that the arithmetic intensity of the DenseGEMMs is severely limited by the number of RHS (ie. the number of problems solved simultaneously.) Therefore traditional DNN accelerators~\cite{eyeriss2016isca,kwon2018maeri,tpu-isca} do not help accelerate these workloads due to fundamentally low reuse.

~\autoref{fig:results}c) shows the arithmetic intensity for one iteration of the CG loop. Please note that for matrix inverse, we consider LU factorization followed by Triangular Solve. Also, we conservatively count accesses to $P$ and $P^T$ separately owing to different layout in the memory. We note that the amount of reuse that can be extracted between the operations is high and this motivates us to design a new dataflow for HPCG workloads which tries to maximize inter-operation rather than optimizing for inter-operation reuse.

\end{comment}

==> Not-here-Arch.tex <==
\section{Accelerator}
\label{sec:arch}

\subsection{Overview}

The Conjugate Gradient accelerator consists of multliple nodes connected via the inter-node interconnect as shown in \TODO{}.

\subsubsection{System Configuration of a Node}

An accelerator node has the configuration close to the AMD Epyc CPU that is used in NVIDIA Selene. The configuration for a single node is shown in ~\autoref{tables:config}.
\input{tables/config.tex}


%\subsection{Matrix Operation Dataflows}

==> algorithm/cg.tex <==
%\vspace{-2mm}
\LinesNotNumbered

\begin{algorithm}
\begin{small}

%\label{algo:inter-op}
\caption{Block Conjugate Gradient. 'prev' and 'cur' stand for previous and current. Only lines with tensor operations inside the loop are numbered.}\label{alg:cg}
$R_0=B-AX_0$\\
$P_0=R_0$\\
$prev=0$\\
\For{iteration=1,2,3...}
{
\nl $S_{prev}=A.P_{prev}$\\
\nl $\Delta=P^{T}_{prev}.S_{prev}$ and $\Lambda=\Delta^{-1}.\Gamma_{prev}$\\
\nl $X_{cur}=X_{prev}+P_{prev}.\Lambda$\\
\nl $R_{cur}=R_{prev}-S_{prev}.\Lambda$\\
\nl $\Gamma_{cur}=R^{T}_{cur}.R_{cur}$\\
\If{$all(diag(\Gamma_{cur})\leq \in)$}
{
    break
}
\nl $\Phi=\Gamma^{-1}_{prev}.\Gamma_{cur}$\\
\nl $P_{cur}=R_{cur}+P_{prev}.\Phi$ \\

$prev=cur$\\
$cur++$\\

}
\textbf{Return} $X_{cur}$
\end{small}

\end{algorithm}

\begin{comment}

  \nl   $S'(m,n)=A(m,k)*P'(k,n)$     \\
 \nl   $\Delta (n,n)=P'^{T}(n,k)*S'(k,n)$ and $\Lambda (n,n)=\Delta ^{-1}(n,k)*\Gamma (k,n)$ \\
 \nl   $X(m,n)=X'(m,n)+P'(m,k)*\Lambda (n,n)$ \\
\nl    $R(m,n)=R'(m,n)-S'(m,k)*\Lambda (n,n)$ \\
 \nl   $\Gamma (n,n)=R^{T}(n,k)*R(k,n)    $  \\
\If{$all(diag(\Gamma)\leq \in)$}
{
    break
}
\nl    $\Phi(n,n)=\Gamma ^{-1}(n,k)*\Gamma (k,n)$ \\
\nl $P(m,n)=R(m,n)+P'(m,k)*\Phi (n,n)$\\

\end{comment}



==> algorithm/cg_einsum_simple.tex <==

\begin{algorithm}
\begin{small}

%\label{algo:inter-op}
\caption{Chain of Einsums for Conjugate Gradient. $k$ represents contractions of size $M$ and $j$ represents contractions of size $N$ and $N'$. Line numbers represent significant computation steps referred to throughout the text.}
\label{alg:cg_einsum}
\KwIn{$A_{m,m}$, $B_{m,n}$, $X_{m,n}$}
$R_{m,n} = B_{m,n} - A_{m,k} * X_{k,n}$ \\
$\Gamma_{n,n}=R_{k,n}*R{k,n}$\\
$P_{m, n} = R_{m, n}$ \\
\While{not converged}
{
  \nl  $S_{m,n} = A_{m,k} * P_{k,n}$     \\
 \nl   $\Delta_{n',n} = P_{k,n'} * S_{k,n}$ and $\Lambda_{n',n} = \Delta^{-1}_{n',j} * \Gamma_{j,n}$ \textcolor{gray}{~~~// $\Delta=P^TS$} \\
 \nl   $X_{m,n} = X_{m,n} + P_{m,j} * \Lambda_{j,n}$ \\
\nl    $R_{m,n} = R_{m,n} - S_{m,j} * \Lambda_{j,n}$ \\
$\Gamma\_prev_{n,n}=\Gamma_{n,n}$\\
 \nl   $\Gamma_{n',n} = R_{k,n'} * R_{k,n}$ \textcolor{gray}{~~~~~~~~// $\Gamma=R^TR$} \\
\If{$all(diag(\Gamma)\leq \epsilon)$} 
{
    \textbf{break}
}
\nl    $\Phi_{n',n} = \Gamma\_{prev}^{-1}_{n',j} * \Gamma_{j,n}$ \\
\nl    $P_{m,n} = R_{m,n} + P_{m,j} * \Phi_{j,n}$
}
\textbf{return} $X$
\end{small}
\end{algorithm}




==> algorithm/interop-backup.tex <==
\vspace{-1mm}
\begin{algorithm}[ht!]
%\label{algo:inter-op}
\definecolor{LimeGreen}{HTML}{32CD32}
\definecolor{BrickRed}{HTML}{AA4A44}
\SetInd{0em}{1em}
\caption{Determination Inter-operation reuse opportunities complete DAG of tensor operations}\label{alg:inter-op}
\begin{footnotesize}

    \For{node $\in$ NODES}
{   
node.numcast=0	\\
\For{edge $\in$ edges(node)}
{
    flag=0\\
    \If{edge.isTransitive == false}{
    node.numcast++\\
    \If{node.numcast > 1}
    {
        \textcolor{LimeGreen}{node.parallel\_multicast=true}
    }
 

}
   \If{node.dominance$\neq$contracted$\And$edge.isTransitive==false}
   {
edge.inter\_dataflow=\textcolor{blue}{pipelineable}
   }
\If{node.dominance==contracted | node.op$\neq$tensor\_mac}
   {
edge.inter\_dataflow=sequential
   }
   \If{edge.dest.dominance $\notin$ edge.tensor.ranks}
   {
edge.inter\_dataflow=sequential
   }
   \If{node.dominance$\neq$contracted$\And$edge.isTransitive==true$\And$ node.pathnext.dominance$\neq$unshared}
   {
\For{pathnode $\in$ longestpath(edge)}
{
\If{pathnode.dominance==contracted or pathnode.pathnext.dominance == unshared}
{edge.inter\_dataflow=\textcolor{BrickRed}{pipeline\_with\_writeback} \\ 
flag=1 \\
break
}
}
\If{flag==0}
{edge.inter\_dataflow=\textcolor{cyan}{pipeline\_with\_hold}
}
   }
}
}

\end{footnotesize}

\end{algorithm}
\vspace{-2mm}


==> algorithm/looporder.tex <==
\setlength{\textfloatsep}{4mm}% Remove \textfloatsep

\vspace{-1mm}
\begin{algorithm}[ht!]
%\label{algo:inter-op}
\SetInd{0em}{1em}
\caption{Determining the loop orders of the tensor operations to exploit reuse}\label{alg:looporder}
\begin{small}

%\emph{Omitted for space. We will purchase an extra page for publication.}

%\begin{comment}

swizzle\_penalty=0\\
    \For{node $\in$ NODES}
{   
 \textcolor{violet}{If the current node doesn't have a dataflow, assign one}\\
 \textcolor{violet}{If operation is not a tensor mul/add, skip to next node.}\\
%node.numcast=0	\\
\For{edge $\in$ edges(node)}
{
    \If{edge.dest.intra\_dataflow==NOT ASSIGNED}{
    %\textcolor{gray}{//Need to assign a dataflow}\\
    \If{edge.inter\_dataflow==\textcolor{blue}{pipelineable} \textbf{or} \\ edge.inter\_dataflow==\textcolor{cyan}{pipeline\_with\_hold}}
    {
        dat=edge.src.intra\_dataflow.loop\_order\\
        \If{dat[0] is contracted}
        {
            print("Loop order doesn't adhere to pipelining")\\
            \textbf{Retry} 
        }
       edge.dest.inter\_dataflow.loop\_order[0]=dat[0]\\
        \textcolor{violet}{Pick the remaining ranks}\\
        \textcolor{violet}{Try a new order if swizzle penalty is high}
    
    }
    \If{node.parallel\_multicast==true}
    {
        \textcolor{violet}{Assign same order to all non-transitive edges}\\
        \textcolor{violet}{First see if a node is already assigned}
        %\If{Loop order wrt multicasted tensor is different}
       % {multicast\_penalty++}
    }
     \If{edge.inter\_dataflow==\textcolor{BrickRed}{pipeline\_with\_writeback} \textbf{or} edge.inter\_dataflow==sequential}
    {
        \textcolor{violet}{Pick an order that does not swizzle}
    }
}
%\textcolor{gray}{//Look for potential inefficiencies}\\
\If{edge.inter\_dataflow==\textcolor{blue}{pipelineable} \textbf{or}\\edge.inter\_dataflow== \textcolor{cyan}{pipeline\_with\_hold}}
{
\If{edge.src.intra\_dataflow.loop\_order[0] is contracted \textbf{or} edge.dest.intra\_dataflow.loop\_order[0] is unshared
}
{
print("Loop order doesn't adhere to pipelining")\\
            \textbf{Retry} 
}
\If{edge.tensor.swizzled}
{
print("Loop order doesn't adhere to pipelining")\\
            \textbf{Retry} 
}
}

 \If{edge.inter\_dataflow==\textcolor{BrickRed}{pipeline\_with\_writeback} \textbf{or}\\edge.inter\_dataflow== sequential}
    {
        \If{edge.tensor.swizzled}
        {
            swizzle\_penalty++
        }
    }

}
}
\If{swizzle\_penalty > $\epsilon$}
{\textbf{Retry}}

%\end{comment}

\end{small}
%\vspace{-1mm}
\end{algorithm}


==> old04-DAG-Dataflow.tex <==
\section{Inter-Operation Reuse Patterns}
%\vspace{-1mm}
\label{sec:dataflows}

This section formulates inter-operation reuse opportunities in the dependency graph of tensor operations using a systematic methodology.
%It formulates a generalized set of inter-operation reuse patterns in an arbitrary dependency graph of tensor operations. 
%We represent the application as a dependency graph, where the node represents an operation and an edge represents the tensor which is the output of the operation represented by the source node and is an input to the operation represented by the desitnation node. 
For the purpose of this paper, the graph is directed and acyclic.

\vspace{-2mm}

\subsection{Generalizing Inter-op reuse patterns}
\label{sec:patterns}

%\TK{As I am readinf through this I realize this sectin is still using the old terminology of ``traditional" rather than ``adjacent-op". @Raveesh can u fix?}

We identify five major inter-operation patterns in an arbitrary tensor DAG. 
%\TK{``There are five .. " or ``We identify five .." ? Also - point to the figure - esp as the color coding matches that, and in each pattern pls point to the figure as example}

\textbf{Sequential} - The sequential pattern executes that particular edge one by one, although it maybe possible to reuse the data on-chip with Sequential pattern depending on the space in the buffer (Note that the term 'sequential' applies to one edge connecting two nodes while we previously defined 'op-by-op' as a configuration computes one op at a time for the entire execution). There are generally no constraints on this type of pattern and this is used when no other pattern is possible. Also, this pattern does not give any benefit, and the output of the operation is both written and re-read from on-chip or off-chip depending on the capacity.

\insertFigure{buffer}{Inter-operation reuse patterns in steady state and their data orchestration.\vspace{-2mm}}
\insertFigure{inter-op-reuse}{Output of~\autoref{alg:inter-op} using colored edges. Letters in the node denote dominance, 'U' means uncontracted, 'C' means contracted and 'bal' means all ranks are moderately big. Note that first tensor is uncontracted dominant since we compress the K rank (CSR format).\vspace{-1mm}}

\textbf{{Adjacent pipeline}} - An adjacent-pipeline reuse pattern refers to pipelining used between the two operations in prior works~\cite{flat,garg2021understanding,tangram,yan2020hygcn}. More than two operations could also be pipelined if more than two consecutive nodes are connected by edges with {adjacent pipeline} patterns.\reviewme{~\autoref{fig:buffer} shows how pipelining reuses the data within SRAM. It discards the tile once its consumed.} For an example pair of Einsums ${Z_{m,n}=\sum_{k}A_{m,k}*B_{k,n}}$ and ${W_{o,n}=\sum_{j}C_{o,j}*Z_{j,n}}$, if the contracted rank in the producer ie. $K$ and the unshared rank in the consumer ie. $O$ are dominant ranks, then pipelining is not beneficial as the producer/consumer needs to wait for several iterations along that dimension. %However, the {pipelineable} pattern does not guarantee pipelining unless additional conditions related to intra-operation dataflow are satisfied which we discuss in~\autoref{sec:gogeta}. 
 Pipelining completely removes the need to write and read the intermediate tensor. However, if the intermediate tensor is needed in the future, there is an additional need to perform {pipeline\_with\_writeback} or {pipeline\_with\_hold}. 


\textbf{{Pipeline\_with\_writeback}} -  Adjacent pipelining completely consumes the intermediate tensor, with the new produced tile replacing the one that has already been consumed. However, the intermediate tensor might be needed in a future computation, a pattern that has not been observed in previously popular applications like Attention, Graph Neural Networks etc. This is represented by the transitive edge (discussed in \autoref{sec:graph}) on the graph. \reviewme{Therefore, as~\autoref{fig:buffer} shows, this tensor needs to be stored in an on-chip SRAM buffer or DRAM depending on the capacity, even though we still avoid reading the tensor for the adjacent operation. }{Pipeline\_with\_writeback} pattern can be seen in CG as~\autoref{fig:inter-op-reuse} shows in brick red color.

\textbf{{Pipeline\_with\_hold}} - As discussed above, we may need a pipelined tensor in the future. But there is a possibility that the complete chain until the future destination of this tensor is pipelineable. \reviewme{In that case, we hold the tile in the SRAM until the destination consumes that tile as~\autoref{fig:buffer} shows.} The number of held tiles essentially depends on the reuse distance of the transitive edge. This pattern provides the full benefit of pipelining but requires slightly more occupancy in the on-chip SRAM. This pattern can be used in ResNet~\cite{resnet} block with skip connections as~\autoref{fig:inter-op-reuse} shows in cyan color.
This work expands the \textit{pipelineable} pattern to mean mean adjacent pipeline, pipeling with hold and pipeling with writeback.

\textbf{{Parallel Multicast}} - It is also possible to reuse the tensor into multiple parallel tensor operations, which we call {Parallel\_multicast}. These parallel operations are non-transitive edges from the multicasting nodes to the directly connected nodes. This can be seen in CG as~\autoref{fig:inter-op-reuse} shows in green color.

\subsection{Node and Edge Attributes of the Graph}
\label{sec:graph}
\vspace{-1mm}
In this section, we discuss the various attributes of the nodes and the edges of the dependency graph that help determine the inter-operation reuse opportunities.

\textbf{node.intra\_dataflow}: Dataflow within the operation that is represented by the node. It consists of loop order, parallelism and tiling strategies.

\textbf{edge.inter\_datflow}: It represents one of the inter-operation patterns in~\autoref{sec:patterns} except {Parallel\_multicast} which is an attribute of the multicasting node and the non-transitive edges are marked automatically if the node is multicasting.

\textbf{node.dominance}: We define dominance in both relative terms and absolute terms since relative terms affect the length of the stage while absolute terms affect the occupancy of the intermediate data. If a rank is greater than 1000 AND the ratio of the rank to the other ranks is more skewed than 100:1, the rank is considered as dominant. This attribute can take four values 'U' (uncontracted rank is dominant), 'C' (contracted rank is dominant), 'bal' (All ranks are not too small and none of them is dominant, minimum value of the rank is 50) and 'small' (all ranks are non-dominant and one of them is less than 50).

\textbf{Critical Path/Longest path}: It is the longest path between first and the last node. Intuitively, its the path that moves forward rather than branching out. $longestpath(edge)$ represents the portion of the critical path between source and destination nodes of that edge.

\textbf{node.pathnext/node.pathprevious}: Next/previous node to/from the current node on the longest path.

\textbf{edge.isTransitive}: This checks whether the edge is transitive or not. A transitive edge is an edge which is not on the critical path but the nodes that it connects are on the critical path. For example, in the CG iteration shown in~\autoref{fig:inter-op-reuse}, both the red edges are transitive edges, since they connect nodes on critical path but are not themselves on it. A transitive edge indicates the output of an operation that will be used later. For a {pipelineable} pattern, transitive edge represents the additional {writeback} or {hold} pattern.  

\textbf{node.numcast}: The number of non-transitive edges originating from the node.

\textbf{node.parallel\_multicast}: Represents that the node has parallel multicast opportunities for its output. All non-transitive edges from the node depict multicasting of the output to multiple operations and are colored green in~\autoref{fig:inter-op-reuse}.

\textbf{edge.src and edge.dest}: Represent the source and the destination nodes of the edge.

\textbf{edge.tensor}: The tensor represented by the edge.

\textbf{node.op}: The operation of the node. Tensor\_mac denotes tensor multiplication or tensor addition/subtraction.

\textbf{edge.tensor.ranks}: Ranks of the edge.tensor

\reviewmehpca{\textbf{Shared rank}: Rank of the intermediate tensor that is the output of the source node and input of the destination node}.

\textbf{edge.tensor.swizzled}: A tensor is swizzled when its read in the opposite order to the order in which it was previously written. For e.g., a tensor $P$ written in M-major order but read in the N-major order is considered swizzled.
%A tensor is also said to be swizzled when the transpose is read in the same order as the tensor. For example, if the tensor $P$ with ranks M,N is written in an M-major order and $P^T$ is also read in the M-major order. 
Swizzling is determined from the relative order of the ranks in the loop order of the source and the destination nodes of the edge. Swizzling of the shared ranks is unacceptable if the inter\_dataflow of the edge is {pipelineable} or {pipeline\_with\_hold}. It incurs a penalty in case of {pipeline\_with\_writeback}. This is further discussed in~\autoref{sec:gogeta}.

\subsection{Inter-Operation Reuse Opportunities}
%\vspace{-1mm}
\input{algorithm/interop.tex}
~\autoref{alg:inter-op} shows the methodology to mark the tensor dependency graph with reuse patterns. A node which has more than one non-transitive edges can multicast its output into more than one parallel operations and thus all the non-transitive edges from that node have the~{parllel\_multicast} pattern. A non-transitive edge where the source node is uncontracted dominant and the destination is unshared dominant has a~{pipelineable} pattern. Note that~{pipelineable} inter-operation pattern does not guarantee pipelining since it also depends on the loop order of the individual operations as we discuss in \autoref{sec:gogeta}. Any edge where the source node is contracted dominant or the destination is unshared dominant, has a sequential inter-operation pattern. A transitive edge with uncontracted dominant source node could have~{Pipeline\_with\_hold} pattern, if all the edges on the corresponding critical path are pipelienable, otherwise it has the~{Pipeline\_with\_writeback} pattern.

%Next, we focus on~\DataflowName mapping strategies for an arbitrary DAG of tensors. %Note, while this graph level formulation in this section is generalizable over all kind of tensor operations of any arithmetic intensity, the next section focusses more on arbitrary DAG of low intensity GEMMs and some of the design decisions are made considering the low intensity of individual GEMMs.


\vspace{-0.5mm}

























\begin{comment}
%\vspace{-1mm}
\section{Insights and Solution}
\label{sec:solution}
%\vspace{-2mm}
\insertWideFigure{results}{Maximum possible Arithemtic Intensity assuming 100\% reuse (Unit is Number of Multiplications/Element Access) for a) SpMM individual operation b) DenseGEMM individual operation c) 1 iteration of CG loop for varying RHS\vspace{-2mm}}

\subsection{Dataflow Considerations}

We explore the various reuse opportunities that CG algorithm offers which would determine the data orchestration.

\subsubsection{Intra-operation Reuse Opportunities}
We saw that reuse opportunities within a operation are less compared to traditional DNNs due to the low arithmetic intensity. Similar to the traditional DNNs, some reuse in the GEMMs can be achieved by using temporally local register files in the PEs or spatially, through multicasting or peer-peer forwarding. Prior works like Alrescha~\cite{asgari2020alrescha} have proposed techniques to extract locality from dense regions of the sparse matrices.

\subsubsection{Inter-operation Reuse Opportunities Within the CG Loop}
Inter-operation reuse can be achieved by reusing the portion of the output of the first operation immediately into the next operation. The design-space of even two of these \textit{pipelined} operations is non-trivial owing to the inter-dependence of the intra-operation dataflows~\cite{garg2021understanding}. However, Conjugate Gradient offers immense pipelining opportunities within one loop iteration of CG Algorithm in ~\autoref{alg:cg_einsum}. Matrix $A$ is the input for every iteration and has to be read once. Every CG loop iteration has dynamically generated matrices $R^{k-1}, P^{k-1}, (R^{k-1})^T, (P^{k-1})^T$ and $X^{k-1}$ as the inputs and $R^k, P^k, (R^k)^T, (P^k)^T$ and $X^k$ as the outputs for the loop. Rest of the intermediate variables (or variable product expressions) are consumed within the single loop iteration. Since, the memory footprint of inputs and outputs to the loop is low, theoretically, the reuse benefit of inter-operation pipelining is high.

\subsubsection{Reuse opportunities between Multiple Iterations of the CG loop}
At an even further granularity, the theoretical reuse across iterations scales. On unrolling the CG for loop $iter$ times, the inputs to a big loop iteration are $A, R^{k-iter}, P^{k-iter}, (R^{k-iter})^T, (P^{k-iter})^T$ and $ X^{k-iter}$ while the outputs are $R^k, P^k, (R^k)^T, (P^k)^T$ and $X^k$. Since all of the input/output variables to the CG loop are dynamically generated and since the only input from the application side $A$ is same across all iterations, the memory accesses in an ideal case are the same regardless of $iter$. Thus maximum achievable arithmetic intensity scales. This kind of a reuse is useful for CG algorithm with RHS=1 and it is achievable due to less memory footprint of that CG algorithm.

%\vspace{-0.5mm}

\subsection{Microarchitectural Considerations}

%vspace{-0.5mm}


There are multiple possible hardware implementations for the dataflows we explore. However, CPUs and GPUs owing to their implicit data orchestration are inefficient since the locality in the HPCG workloads is poor. Moreover, the inter-operation data communication would happen through the memory hierarchy which is expensive.

Spatially programmed accelerators (or Dataflow Accelerators) on the other hand enable efficient pipelining since they convert these cache accesses into direct communication. However, within, spatial accelerators, large fixed dataflow DNN acceelrators like Google TPU~\cite{tpu-isca} and NVDLA~\cite{nvdla} are optimized for intra-operation reuse which is low in the HPCG workloads. We aim to propose a substrate with small reconfigurable GEMM engines for individual operation execution and focus on the buffer hierarchy and interconnect that optimizes inter-operation communication.

Using programmable scratchpads would allow us to have flexible partitions for various variables and would also allow a more explicit control over the data orchestration~\cite{buffets}. Moreover, support for ping-pong buffering at various granularities would enable us coarse-grained pipelining in addition to the fine-grain pipelining and would also allow access of certain variables used in multiple iterations, for example, $R^{k-1}$ which are required even after $R^k$ is generated.

%\vspace{-1mm}

\subsection{Conjugate Gradient Algorithm Variants}
We also plan to support variants of conjugate gradient algorithm, for example Pre-conditioned conjugate gradient algorithm an  (PCG)~\cite{bramble1988preconditioning} which uses pre-conditioning to achieve faster convergence and BiCGStab~\cite{van1992bi} which extends conjugate gradient to non self-adjoint $A$ matrices.

\end{comment}

==> old05-Gogeta.tex <==

%\input{algorithm/looporder.tex}
\section{GOGETA Mapping}
\label{sec:gogeta}
\vspace{-1mm}
In this section, we determine the dataflows and tile sizes of individual operations, given that the dependency graph is marked with inter-operation reuse patterns. Through this, we determine the entire mapping which we call~\DataflowName.

%\input{tables/inter_equations.tex}
%\insertWideFigure{inter-op}{(a) Algorithm for dynamic determination Inter-operation reuse opportunities for every edge in the DAG of tensor operations and the output of the algorithm shows colored edges. Letters inside the node denote dominance and 'bal' means all ranks are moderately big. Note that first tensor is M dominant since we compress the K rank (CSR format). (b) Algorithm to determine the loop orders of the tensor operations to exploit reuse.}




%\insertWideFigure{spacetime-dist}{Space-time representation of an iteration of Conjugate Gradient with loop orders. The tensors are split across the node by the dominant rank and the sub-tensors are pipelined within a cluster. This is the set of loop orders with zero swizzle penalty.}
\insertFigureScaled{spacetime}{Example space-time representation of an iteration of CG loop orders with zero swizzle penalty. In the top chart, the overall compute is divided into multiple parts each executing one tensor. In the bottom chart, the tensors are split across the node by the dominant rank and the sub-tensors are pipelined within a cluster. See~\autoref{alg:cg_einsum} for rank names. 
%$M$ represents the large rank, $N$ ($\equiv N'$) represents the small ranks. $K$ represents contractions of size $M$ and $J$ represents contractions of size $N$.
\vspace{-3mm}}{0.85}
%\vspace{-2mm}

\insertFigure{tornado}{Data organization in the scratchpad. Top shows scratchpad filling up without replacement. The part that could not fit is sent to DRAM. Bottom part shows that after queue is filled, the tail of $X$ is evicted and next element of $R$ is enqueued at the head to fill the space.\vspace{-2mm}}

\subsection{Loop order and Layouts}
\label{sec:loop}

In this section, we systematically determine the loop orders of the individual tensors after the inter-operation reuse patterns have been marked as a result of~\autoref{alg:inter-op}.  We determine the loop orders to make sure that we are able to pipeline wherever the inter-operation reuse pattern is pipelineable, which is important for low AI individual operations, and we retry with a new set of loop orders if a pipelineable edge cannot be pipelined due to the loop order pair of the source and the destination nodes.
This constraint could be relaxed into a penalty rather than having to retry for workloads which have higher intensity GEMMs.

For an example pair of Einsums $Z_{m,n}=\sum_{k}A_{m,k}*B_{k,n}$ and ${W_{o,n}=\sum_{j}C_{o,j}*Z_{j,n}}$. The conditions for pipelining a loop order pair are as follows-
%\vspace{-2mm}
\squishlist
\item The edge connecting the nodes has a {pipelineable} inter-operation pattern.
\item The source node has an uncontracted rank as the outermost loop. Having contraction ($K$) as the outermost loop implies that the complete sum that is usable by the next operation is generated at the very end.
\item The destination node has a shared rank as the outermost loop. Having unshared rank ($O$) as the outermost loop implies that the shared tensor $Z$ is needed all over again when $o$ changes. But the idea of pipelining is to slice the intermediate tensor and consume it so that its not needed.
\item The shared tensor $Z$ is not swizzled since the same portion of data that is produced, should be consumed. %Thus no swizzling at that edge is allowed.
\squishend


The algorithm ensures that each of the edges with {adjacent pipeline} and {pipeline\_with\_hold} patterns have compatible loop orders. For {parallel multicasting}, the loop orders of all consumer nodes should be the same.
%TODO RE-ADD FOR CAMERA READY
%The algorithm assigns the dataflow to the node with no assignment yet, based on pipelining and multicasting conditions.
%It also checks whether those conditions are met in case the dataflow was already assigned by some other incoming edge. 
%It returns a retry if a pipelineable edge cannot be pipelined due to a certain loop order pair.
In the {Pipeline\_with\_writeback} and Sequential case, it increases the penalty in case a tensor is swizzled. If the swizzle penalty exceeds a threshold $\epsilon$, then the algorithm retries. In the end, a set of loop orders with all or maximum possible pipeline friendly edges and minimum swizzle penalty is selected. %This threshold, could start from zero and gradually increase if we don't find a set of loop orders.

For CG, we determine a set of loop orders (shown in~\autoref{fig:spacetime}) 
%These 
%orders 
%have 
with zero swizzle penalty with pipeline conditions satisfied. %and parallel\_multicasted operations having same order wrt the multicasted tensor $\Lambda$ which is $MKN$ ie $P-$stationary and $S$-stationary respectively.

\subsection{Tiling Strategy}
\label{sec:tiling}

\textbf{Individual GEMMs}: There are limited options for tiling individual low intensity \GEMM because the non-dominant dimensions are small. In fact such GEMMs are often able to achieve the best possible data reuse with memory accesses $MK+KN+MN$ since the tensor made of the non-dominant ranks (for e.g., $\Lambda$ in line 3 and 4 of~\autoref{alg:cg_einsum} and $\Gamma$ in line 5) can practically fit inside a portion of the Register File (RF) or parallelized across few PEs which means that the smaller tensor can just be accessed continuously from the RF while a tile of the large tensor is stationary. However, as discussed in~\autoref{sec:ai}, even the best intensity is low for \GEMM.

\textbf{Considering multiple GEMMs}: With pipelining and parallel\_multicast, there are different ways in which data can be communicated spatially. Assuming multiple clusters of sub-accelerators, one could pipeline by having the whole tensor be local and occupy the two halves of compute entirely. Prior works like~\cite{simba,tangram} have divided the substrate into large chunks for each tensor just like~\autoref{fig:spacetime} top shows. The major disadvantage of that would be a significant sized tensor being communicated through the inter-cluster NoC which usually has lower bandwidth than the intra-cluster NoC. On the other hand, for skewed GEMMs, which do not have significant intra-operation reuse anyway, we propose to slice the dominant rank on multiple clusters instead and have the tensors be pipelined within a cluster as~\autoref{fig:spacetime} bottom shows. When the dominant rank is split ($M$ for example in line 4 of~\autoref{alg:cg_einsum}) the chunks would share the small tensor formed by non-dominating ranks($\Lambda$) and $\Gamma$. Broadcasting $\Lambda$ and reducing $\Gamma$ on the inter-cluster NoC has orders of magnitude less communication on the inter-cluster NoC compared to communicating $R$ between clusters.

\reviewmehpca{As an example, if we consider operations 4 and 5 in CG~(\autoref{alg:cg_einsum}), the total traversals on the inter-cluster NoC, obtained by dividing the total compute into contiguous chunks and mapping operations on them (\autoref{fig:spacetime} up) is $sizeof(R)$ which is $M\times N$ even if these operations are allocated such that they are 1 hop apart which leads to considerable delay and energy since inter-cluster bandwidth ($\equiv$ inter-chiplet) is low compared to in-cluster bandwidth. Instead, if we use considered the tiling strategy proposed in~\autoref{sec:tiling} and where pipelining happens inside the cluster and $M$ rank is sliced across the clusters (\autoref{fig:spacetime} down), maximum inter-cluster link traversals are $sizeof(\Lambda)\times Broadcast~traversals$ + $sizeof(\Gamma)\times Reduce~traversals$ which is $2\times N\times N\times 15$ ($N\times N$ data moved through at most 15 links for broadcast and reduction) for 16 clusters. Given that M is the dimensions that scale with larger workloads, this tiling strategy can prevent proportional increase of communication traffic in potentially large systems with even off-chip networks.}



\subsection{Custom Scratchpad Management}
\label{sec:tornado}
\vspace{-1mm}
There are various scenarios regarding the amount of tensors the scratchpad can hold ranging from a fraction to multiple tensors depending on the workload size and the architecture. In \DataflowName, we choose the loop orders to minimize the swizzling of ranks in a tensor and hence the tensor will be read in the same order as it was written. Due to this, we write the tensor in the queue order and if the scratchpad is full, we send the remaining portion of that tensor directly to DRAM as~\autoref{fig:tornado} shows. We call this \textsc{Qpad} for the purpose of evaluation. This makes sure that we access the portion of the tensor in the scratchpad first rather than replacing it by the later part of the tensor and again reading the earlier part. This is in contrast to the various buffer management schemes that keep the recently accessed data. If the tensor fits, we repeat this for multiple operations. We read the tensor at head.

While this makes sure that we minimize the off-chip traffic for that particular tensor, there is still a chance that a particular tensor which is not reused until later (for example, $X$ in line 3 of~\autoref{alg:cg_einsum} which is used in line 3 of the next iteration) is written to scratchpad at the expense of a future tensor that is used before the reuse of the previous tensor (for example $R$ in line 4 which is reused in lines 5 and 7 of the same iteration). In that case, based on the reuse distance, we prioritize $R$ and evict out a portion of $X$ to make room for $R$ by evicting the later elements of $X$ first. Then $R$ is read at its head. This is the first work to the best of our knowledge that considers reuse distance and frequency of a tensor in the dependency graph and proposes data organization strategies at a tensor granularity. We call this \textsc{FDpad} (Frequency and Distance).

If 3 and 4 were executed in parallel as~\autoref{fig:spacetime} shows, $R$ and $X$ would occupy equal halves in the second step and the later part of $R$ will eventually replace the tail of earlier part of $X$ and the later part of $X$ would be sent straight to DRAM, resulting in the same proportions of $R$ and $X$.


























\begin{comment}
\subsection{Loop Optimizations for operation pipelining}

For operation pipelining to work, the order of production and the order of consumption of data should be the same and the contracted rank should not be the outermost loop of the first operation and the rank exclusive to second operation should not be the outermost loop of the second operation~\cite{garg2021understanding}.
For example, between $S=AP$ and $var=P^TS$, matrix $S$ is $M\times N$ for the first operation and $K\times N$ for the second operation. $MNK\xbottomarrow{}KNM$ is valid loop order pair since the dimensions corresponding to S are in the outer loop and are in the same row major order. $KNM\xbottomarrow{}MNK$ is an invalid loop order pair for pipelining since contracted rank on the outermost loop of the first operation implies that the actual output of the first operation is produced in the end and the outermost M on second operation implies that the all outputs of the first operation need to be available every time M changes in the second operation, negating the benefit of pipelining.

Moreover, splitting the higher rank enables a finer grained pipelining, thus this work considers the biggest rank to always be the outermost loop as shown in ~\autoref{fig:spacetime} loop orders.

Moreover, balancing the production rate and consumption rate is necessary for operation pipelining. For example, between $S=AP$ and $var=P^TS$, matrix $S$ is $M\times N$ for the first operation and $K\times N$ for the second operation, tile sizes $M0_{operation 1}=K0_{operation 2}$ and $N0_{operation 1}=N0_{operation 2}$ will ensure fine grained operation pipelining without the need to take LCM~\cite{garg2021understanding}.

For a continuous pipelining between the tensor operations, the biggest ranks should ideally be the uncontracted ranks since the high contracted rank requires significant portion of compute to just produce the output in the first place.
However, in the Conjugate Gradient Algorithm, operations 2 and 5 have contracted rank (K) as the dominant rank due to which they do not provide benefit of fusing further. 
Therefore, for the loop of  we fuse lines (1,2a($var={P_{prev}}^TS_{prev}$)); (4,5) and parallelize 3 and 4 since the output of operation 2, $\alpha$, branches into operations 3 and 4 and can be multicasted. The space time representation of kernels is shown in ~\autoref{fig:spacetime}. Please note that operations 2b ($\alpha_{prev}=var^{-1}\gamma_{prev}$) and 6 have all small ranks thus have negligible compute and memory footprint compared to other operations. We discuss the individual phase dataflow in more detail along with the accelerator architecture in ~\autoref{sec:arch}.

\section{Generalizing Inter-Operation Reuse}

\subsection{Limitations of treaditional operation pipelining}
%\RG{move in the intro, give a hint of next}

Operation pipelining can significantly reduce the data movement between multiple operations in the following situations:
\squishlist
\item For applications with tensor operations where the all the matrix ranks are large enough specially the non-contracted rank. For example, in Deep Learning, batch size is a non-contracted rank and the operation pipelining can be done by splitting batches into stages. Also, deep learning has relatively large number of input and output features.

\item For applications where the arithmetic intensity of tensors is low and the dominant rank is \textit{always} the non-contracted rank.

However, operations with contracted rank as the dominant rank do not result in significant data movement reduction due to operation pipelining since a significant number of operations and data movement is needed to just generate the output matrix. Examples of this include operations 2a and 5 of the Conjugate Gradient algorithm.

%\insertFigure{dfg-analysis}{Tensor dependency graphs of some applications with fusion opportunities. Letters inside the node represent the dominant rank in case of a low intensity operation. 'Bal' means that all ranks are somewhat large. Please note that in a) annd b), we assume that the first operation follows the CSR format where MK is the sparse matrix and K rank is compressed, which makes M the dominant rank.}

~\autoref{fig:inter-op} shows examples of applications where \textit{traditional operation pipelining} works and applications where it does not work. Conjugate Gradient does not offer benefit of pipelining the entire graph because of operations with dominating contracted ranks. A single layer of GNNs supports pipelining since M is the dominant rank in both the operations assuming sparse phase is executed first. Similarly, ResNet allows pipelining of all the operations inside the residual block, this is typically done by batch since batches are non-contracted ranks in all the operations. Prior works like TANGRAM~\cite{tangram} and SIMBA~\cite{simba} pipeline operations in the block. In certain cases, the arithmetic intensity of an operation might be high such that it offers better reuse opportunities within the operation.

Therefore, based on (1) tensor dependency graph (2) Shape and Arithmetic Intensity of the operations, we determine whether pipelining is required and whether traditional pipelining is possible or if writeback is required.

\squishend
\subsection{Beyond Pipelining: Tensor Reuse Distance}



\end{comment}


\reviewme{\subsection{Architectural Support}
\label{sec:arch_implications}

\autoref{fig:spacc} shows the architecture of a flexible spatial accelerator~\cite{eyeriss2016isca,plasticine,kwon2019understanding,flexagon,kwon2018maeri,sigma} that we use in our evaluations.
We describe the key features needed in an accelerator to be able to  run GOGETA mappings. 

\textbf{Flexible Dataflow.} 
GOGETA relies on an accelerator being able to run individual GEMM operators, both dense and sparse, with any dataflow (i.e., loop orders and parallelism) and diverse tile sizes, as discussed earlier in \autoref{sec:loop} and \autoref{sec:tiling} respectively. For instance, CG contains a contracted dominant GEMM which requires tiling both inputs and large parallel reduction, and an uncontracted dominant GEMM which requires tiling one input and one output and large parallel input broadcast.
%
Several prior accelerators~\cite{eyeriss2,kwon2018maeri,sigma,flexagon} have demonstrated the required support within the interconnect and scratchpads to run diverse dataflows. Specifically, support for broadcast and reductions within the interconnect, and programmable address generators for the scratchpad can allow any dataflow to be orchestrated~\cite{flexion}. 
Further, leveraging fully addressable buffers allows for picking diverse tile sizes. 
%
In this work, we select Flexagon~\cite{flexagon} as the baseline accelerator, as it is the most recently published work in this line of research, and can in principal, support flexible dataflows for both dense and sparse GEMM operators. However, recall that, Flexagon, and almost all prior works, run the individual operators in op-by-op manner, as discussed before in \autoref{sec:background}.

\textbf{Addressable Scratchpad.} 
Beyond the dataflow (\autoref{sec:loop}) and tile sizes (\autoref{sec:tiling}), GOGETA's proposed scratchpad management techniques can either be implemented in HW via custom buffers, or implemented in SW over a fully programmable scratchpad. While the former is certainly expected to be more area efficient, it limits the applicability of the accelerator to only support a certain set of workloads that may use \DataflowNamenospace. In this work, we model the latter. 
Several commercial accelerators today~\cite{tpuv4,cerebras,sambanova}
%like TPUv4~\cite{tpuv4}, Cerebras\cite{cerebras}, SambaNova~\cite{sambanova} 
provide such programmable scratchpads already. \textsc{Qpad} can be implemented by writing to consecutive addresses until the SRAM is full, and implement the \textsc{FDpad} strategy by overwriting on the addresses where the previous tensor needs to be replaced.
}
%{\color{red} @Raveesh -- what does ``end" mean in the prev sentence. Might be good to elaborate a bit more}

\insertFigure{spacc}{Cannonical spatial accelerator. We focus on one compute node. A cluster could be a sub-accelerator~\cite{kwon2021heterogeneous} or chiplet~\cite{simba}.\vspace{-2mm}}

==> old06-Methodology-new.tex <==
%   \reviewme{\subsection{Architectural Implications}


\section{Evaluations}

\subsection{Experimental Methodology}
\label{sec:expt}

We describe our experimental methodology for demonstrating the efficiency of \DataflowName across baseline dataflows.
%\vspace{-2mm}


%\indent \textbf{Analytical Framework:~}
%\label{sec:simulation}
%We modify the OMEGA~\cite{garg2021understanding} framework to model the DAG of tensor operations for applications like Conjugate Gradient, Graph Convolution Networks, ResNet. OMEGA is a cost model for modelling performance and energy for various mappings with two-operation pipelining.
%Our framework builds upon STONNE~\cite{STONNE21} which is a cycle accurate simulator that models one DNN layer at a time and models flexible interconnects~\cite{kwon2018maeri} with ability to support multiple intra-operation dataflows. STONNE has been extensively validated against MAERI~\cite{kwon2018maeri} and SIGMA~\cite{sigma} RTLs. STONNE can model SpMM, DenseGEMMs/CONVs on the accelerator with reconfigurable interconnects. Prior work OMEGA~\cite{garg2021understanding} builds a cost model which uses the STONNE output and timestamps to model pipelining between two operations. We modify the cost model that OMEGA uses to model a DAG of tensors in applications like Conjugate Gradient. We use that to simulate the baselines and \DataflowName which are described in~\autoref{sec:baseline}.

\reviewme{\textbf{Modeling Framework.}
%\label{sec:simulation}
We developed an analytical framework to model the DAG of tensor operations for applications like Conjugate Gradient, GNNs, DNNs (e.g., ResNets) and schedule the operators in an op-by-op manner or via all the pipelined schemes introduced in this work. For each operator, we determine the best intra-operator dataflows and tile sizes (using individual operation tiling strategies in~\autoref{sec:tiling}) to maximize compute utilization.
%This dataflow search is similar to the one employed by mappers in MAESTRO~\cite{chatarasi2020marvel} and Timeloop~\cite{timeloop}.
%, assuming a flexible dataflow accelerator. 
Next, we leverage \DataflowName to determine the inter-operator mapping.
%We then schedule the operators over an accelerator simulated using STONNE~\cite{STONNE21}, which is a cycle accurate simulator for flexible dense and sparse dataflow accelerators, including our baseline Flexagon~\cite{flexagon}\footnote{\reviewme{The reason to pick STONNE, rather than an analytical cost model~\cite{timeloop} is due to its support for sparse inputs.}}.
Our framework captures the memory acceseses through the hierarchy and communication over the NoC across all the mapping strategies. DRAM accesses for individual operations are validated using the STONNE cycle-accurate simulator~\cite{STONNE21}. Our framework also computes the arithmetic intensities from the DRAM accesses and the throughput using the equations in~\autoref{sec:roofline}, which we use to plot gaps from ideal in our results. 
%We plot the throughput of all the data points and expand the last one into a roofline showing both throughput and arithmetic intensity. We also plot reduction in DRAM accesses and sensitivity studies on inter-cluster NoC communication and change in memory bandwidth (\autoref{fig:comm}).
}


% We developed an in-house analytical model to capture the memory accesses and communication across an accelerator's memory hierarchy. We validated per-layer statistics against STONNE~\cite{STONNE21}, which is a cycle accurate simulator that models one operation (it can model GEMM, SpMM, SpMSpM, CONV) at a time. 
% STONNE also models our baseline flexible accelerator Flexagon~\cite{flexagon}.

% We build an analytical model to capture the memory accesses and communication across clusters for the baselines and \DataflowName to compare the achieved arithmetic intensity of the dataflows independent of the accelerator implementation. We validate the DRAM statistics for a single layer by using STONNE~\cite{STONNE21}, which is a cycle accurate simulator that models one operation (it can model GEMM, SpMM, SpMSpM, CONV) at a time. STONNE can be supplied with various dataflows and tile sizes as inputs. STONNE also models the flexible accelerator Flexagon~\cite{flexagon}. We model SpMM (the sparse matrix is in CSR format) and GEMM the microarchitecture of Flexagon since it is Flexible enough to support any mapping to get a strong op-by-op baseline. %We validated the data movement for a pair of two pipelined tensor operations using OMEGA~\cite{garg2021understanding,omega} which is a wrapper around STONNE to model pipelining between two operations. 

\input{tables/config.tex}
\input{tables/workload.tex}

\input{tables/dataflow_config.tex}
\label{sec:dataset}

\reviewme{\textbf{Architecture Parameters}
\label{sec:arch} 
We consider a clustered architecture, each cluster of 1024 PEs connected using a NoC, backed by its own SRAM slice, as shown in \autoref{fig:spacc}. We sweep different SRAM capacities and memory bandwidths as shown in \autoref{table:config} . Together with diverse tensor sizes across workloads and datasets, this allows us to study the efficacy of \DataflowName across diverse tensor shapes and sizes.} 

\indent \textbf{Workloads and Datasets:~} 
\autoref{table:dataset} shows the workloads and the datasets.
We obtain the sparse matrices of the CG datasets from Suitesparse~\cite{suitesparse} for scientific problems like structural problems, circuit simulation, and so on. For CG, we also sweep the $N$ rank that corresponds to number of simultaneous initial guesses, as shown in \autoref{table:config}. 
We obtain GNN graphs from OMEGA~\cite{omega}.
We run workloads of different sizes and nnz's. We also evaluate ResNet and SSD ResNet.%{\color{red} @Raveesh -- the table also shows params for Attention layer now. Might be good to simply point to the table sayin we vary different params across workloads to save space}




% \indent \textbf{Workload and Architecture Parameters:~}
% \autoref{table:config} describes the architecture configuration we use for the evaluation and the parameters we sweep. We run workloads of different sizes and nnz's and we also sweep the $N$ rank that corresponds to number of simultaneous initial guesses and the SRAM size to capture different scenarios with varying ratios of tensor and SRAM sizes. In some cases, tensors are either too small or too large for the SRAM and in some cases, a varying proportions of tensors can fit.
% We consider a clustered architecture, each cluster of 1024 PEs backed by its own SRAM slice.

\label{sec:baseline}



\indent \textbf{Dataflow Configurations:~}
%\TK{Note to self -- we should be able to shorten this .. is repeating what table IV says}
We compare multiple dataflow configurations described in~\autoref{table:dataflow_config}. 
We evaluate all schemes over the same HW substrate (\autoref{sec:arch_implications}) to isolate the effects due to the mapping instead of microarchitectural effects.

\begin{comment}
Flexagon-like dataflow models an oracle operation-by-operation dataflow, running SpMM and~\GEMM on the flexible microarchitecture.
%It is able to achieve the lowest possible DRAM accesses for individual operations, but it requires the output tensor of each operation ending up in the DRAM and the input coming from the DRAM.}
%
%Flexagon-like dataflow is modelled based on the microarchitecture of Flexagon~\cite{flexagon}. We model SpMM and~\GEMM on the flexible microarchitecture. It is able to achieve the lowest possible DRAM accesses for individual operations but it considers the output tensor of each operation ending up in the DRAM and the input coming from the DRAM. Its the oracle operation-by-operation dataflow. 
%
Adjacent pipeline baseline consists of situations where only adjacent pipeline is possible and any kind of dependency that results in writeback or hold results in sequential execution. We demonstrate that in CG, adjacent pipeline cannot be applied while it can be applied in GNN layer and only part of ResNet layer.
\DataflowNamenospace-\textsc{Qpad} does not consider pipelining, however, it writes the portion of the tensor that fits in the scratchpad in FIFO order proposed in~\autoref{sec:tornado} but does not consider distance/frequency based replacement. This ensures that parts of intermediate tensors that could fit, are still reused inside the SRAM. \DataflowNamenospace-\textsc{Qpad} by itself does not minimize swizzle penalty, it still writes the data in FIFO manner for tensors that are not swizzled later.
%
\DataflowNamenospace-\textsc{all} uses all the contributions proposed.
%It uses the inter-op patterns proposed in~\autoref{sec:dataflows} and finds the individual loop orders which enable pipelining and avoid swizzle\_penalty proposed in~\autoref{sec:loop} and also uses the scratchpad management in~\autoref{sec:tornado}. It also uses scalable tiling strategy that reduces inter-cluster communication overhead proposed in~\autoref{sec:tiling}.

Ideal, represents the arithmetic intensity with perfect reuse and infinite SRAM capacity.
\end{comment}

\label{sec:params}

\insertFigure{AI}{Throughput for CG workload for first 10 iterations of the CG loop. Memory BW = 1000 GB/s. We sweep the SRAM capacity - \{1MB, 4MB, 16MB\}. N=\{1,16\} and is mentioned in parenthesis as (1)/(16) along with the dataflow configuration. \reviewme{At the bottom, we show the dataset-wise geomean throughput gain of \DataflowName \textsc{all} over Flexagon-like. We also show the last chart on a roofline.}\vspace{-3mm}}

\insertFigure{GNN}{Throughput for GNNs and ResNets\vspace{-1mm}}

\insertWideFigure{comm}{(a) Normalized DRAM access reduction for each dataflow configuration geomeaned across workload and architecture configurations.
(b) Inter-cluster link traversals in KBs for N=8. (c) Effect of Memory BW on throughput}
%\insertFigure{Energy}{Normalized DRAM accesses for each dataflow configuration geomeaned across all workload and architecture configurations. This directly impacts the energy.\vspace{-1mm}}
%\insertFigureRevision{bert}{Roofline plots for attention layers.}

% \indent \textbf{Workload and Architecture Parameters:~}
%\autoref{table:config} describes the architecture configuration we use for the evaluation and the parameters we sweep. We run workloads of different sizes and nnz's and we also sweep the $N$ rank that corresponds to number of simultaneous initial guesses and the SRAM size to capture different scenarios with varying ratios of tensor and SRAM sizes. In some cases, tensors are either too small or too large for the SRAM and in some cases, a varying proportions of tensors can fit.
%We consider a clustered architecture, each cluster of 1024 PEs backed by its own SRAM slice.


==> old06-Methodology.tex <==
\section{Evaluations}

\subsection{Experimental Methodology}
\label{sec:expt}

We describe our experimental methodology for demonstrating the efficiency of \DataflowName across baseline dataflows.
%\vspace{-2mm}
\indent \textbf{Analytical Framework:~}
\label{sec:simulation}
%We modify the OMEGA~\cite{garg2021understanding} framework to model the DAG of tensor operations for applications like Conjugate Gradient, Graph Convolution Networks, ResNet. OMEGA is a cost model for modelling performance and energy for various mappings with two-operation pipelining.
%Our framework builds upon STONNE~\cite{STONNE21} which is a cycle accurate simulator that models one DNN layer at a time and models flexible interconnects~\cite{kwon2018maeri} with ability to support multiple intra-operation dataflows. STONNE has been extensively validated against MAERI~\cite{kwon2018maeri} and SIGMA~\cite{sigma} RTLs. STONNE can model SpMM, DenseGEMMs/CONVs on the accelerator with reconfigurable interconnects. Prior work OMEGA~\cite{garg2021understanding} builds a cost model which uses the STONNE output and timestamps to model pipelining between two operations. We modify the cost model that OMEGA uses to model a DAG of tensors in applications like Conjugate Gradient. We use that to simulate the baselines and \DataflowName which are described in~\autoref{sec:baseline}.
We build an analytical model to capture the memory accesses and communication across clusters for the baselines and \DataflowName to compare the achieved arithmetic intensity of the dataflows independent of the accelerator implementation. We validate the DRAM statistics for a single layer by using STONNE~\cite{STONNE21}, which is a cycle accurate simulator that models one operation (it can model GEMM, SpMM, SpMSpM, CONV) at a time. STONNE can be supplied with various dataflows and tile sizes as inputs. STONNE also models the flexible accelerator Flexagon~\cite{flexagon}. We model SpMM (the sparse matrix is in CSR format) and GEMM the microarchitecture of Flexagon since it is Flexible enough to support any mapping to get a strong op-by-op baseline. %We validated the data movement for a pair of two pipelined tensor operations using OMEGA~\cite{garg2021understanding,omega} which is a wrapper around STONNE to model pipelining between two operations. 

\input{tables/workload.tex}
\label{sec:dataset}

\indent \textbf{Workloads and Datasets:~}
We evaluate our methodology and the \DataflowName mapping strategy for Conjugate Gradient and GNN. We obtain the sparse matrices of the Conjugate Gradient Datasets from Suitesparse~\cite{suitesparse} for scientific problems like structural problems, circuit simulation, etc. We obtain GNN graphs from OMEGA~\cite{omega}.~\autoref{table:dataset} shows the workloads and the datasets.

\label{sec:baseline}
\input{tables/dataflow_config.tex}

\indent \textbf{Dataflow Configurations:~}
We compare multiple dataflow configurations described in~\autoref{table:dataflow_config}. Flexagon-like dataflow is modelled based on the microarchitecture of Flexagon~\cite{flexagon}. We model SpMM and~\GEMM on the flexible microarchitecure. It is able to achieve the lowest possible DRAM accesses for individual operations but it considers the output tensor of each operation ending up in the DRAM and the input coming from the DRAM. Its the oracle operation-by-operation dataflow. 

\DataflowNamenospace-\textsc{Qpad} does not consider pipelining, however, it writes the portion of the tensor that fits in the scratchpad in FIFO order proposed in~\autoref{sec:tornado} but does not consider distance/frequency based replacement. This ensures that parts of intermediate tensors that could fit, are still reused inside the SRAM. \DataflowNamenospace-\textsc{Qpad} by itself does not minimize swizzle penalty, it still writes the data in FIFO manner for tensors that are not swizzled later.

\DataflowNamenospace-\textsc{all} uses all the contributions. It uses the inter-op patterns proposed in~\autoref{sec:dataflows} and finds the individual loop orders which enable pipelining and avoid swizzle\_penalty proposed in~\autoref{sec:loop} and also uses the scratchpad management in~\autoref{sec:tornado}. It also uses scalable tiling strategy that reduces inter-cluster communication overhead proposed in~\autoref{sec:tiling}. Ideal, represents the arithmetic intensity with perfect reuse and infinite SRAM capacity.

\label{sec:params}

\input{tables/config.tex}


\indent \textbf{Workload and Architecture Parameters:~}
\autoref{table:config} describes the architecture configuration we use for the evaluation and the parameters we sweep. We run workloads of different sizes and nnz's and we also sweep the $N$ rank that corresponds to number of simultaneous initial guesses and the SRAM size to capture different scenarios with varying ratios of tensor and SRAM sizes. In some cases, tensors are either too small or too large for the SRAM and in some cases, a varying proportions of tensors can fit.
We consider a clustered architecture, each cluster of 1024 PEs backed by its own SRAM slice.


==> old07-Evaluation.tex <==
\vspace{-2mm}
\subsection{Results}
\vspace{-1mm}
\label{sec:eval}

\indent \textbf{Throughput for Conjugate Gradient:~}
We model the substrate and sweep the parameters as discussued in~\autoref{sec:expt} for the CG workloads and datasets in~\autoref{table:dataset}, and plot the throughput
%, SRAM accesses and memory footprint of operations
in ~\autoref{fig:AI}.
We expand the last plot to a roofline showing both AI and throughput.
\DataflowNamenospace -\textsc{all} achieves a \reviewme{geomean of 5.97x improvement in AI over the Flexagon-like baseline, ranging from 1.34x to 23x}. This translates to geomean 5.25x improvement in throughput.

We discuss key observations and insights next.
In CG, all the tensors that can be pipelined also have a delayed consumer and as a result, the adjacent pipelining baseline cannot overwrite the fan out tensor as that will violate the later dependency, thus showing same performance as op-by-op (i.e., Flexagon-like).

\reviewme{For a dataset with tensors smaller than the SRAM size for example, fv1 and nasa4704 at 4 and 16 MB SRAM}, \DataflowNamenospace -\textsc{all} and \DataflowNamenospace -\textsc{Qpad} achieve the peak throughput, which is orders of magnitude more than the Flexagon and adjacent pipeline baselines.

\reviewme{For large datasets like G2\textunderscore Circuit, for small memory size, Flexagon-like and \DataflowNamenospace -\textsc{Qpad} have the similar AI and \DataflowNamenospace -\textsc{all} achieves roughly 30 to 50\% better throughput} than them due to pipelining\_with\_writeback which avoids reading the operand from the DRAM for the consecutive operation. However, given 16MB SRAM size, G2\textunderscore Circuit, it can show better improvement with N=1. Though large datasets are not executed on a single compute node and are often distributed on machines. We also show the communication reduction, \DataflowNamenospace -\textsc{all} can achieve due to tiling in~\autoref{fig:comm}. 

For all the intermediate data points, where SRAM is neither too large and nor too small, there is a clear upward trend between Flexagon-like(=Adjacent pipelining), \DataflowNamenospace -\textsc{Qpad} and \DataflowNamenospace -\textsc{all} in terms of throughput. This is due to a combination of multiple reasons, including pipelining\_with\_writeback, scratchpad management based on reuse distances of downstream tensor operations and the ability to achieve zero swizzle penalty with~\DataflowName.



%\reviewme{To summarize, we show geomean improvement in \DataflowNamenospace -\textsc{all} over Flexagon-like dataflow for each dataset in~\autoref{fig:AI}}

%\input{tables/geo}

Thus \DataflowNamenospace -\textsc{all} achieves the best performance due to pipelining, swizzle aware loop ordering and due to scratchpad management strategies.
%We also evaluate DRAM accesses for Graph Neural Networks  in~\autoref{sec:GNN} to demonstrate the generality of \DataflowName.
%For Conjugate Gradient, we evaluate 10 iterations, for GCNs, 1 layer and for ResNet, we evaluate one residual block.% We also compare inter-cluster communication between GOGETA-df and GOGETA-map to demonstrate the benefit of pipelining with fine-grained spatial multiplexing. %We also evaluate a set of loop orders with loop orders that support pipelining but incur swizzling. 

%\TK{@Raveesh -- need to highlight following points: geomean speedup, impact of sram size, and how far you are from ideal}
%\vspace{-.5mm}
%\subsubsection{Roofline Analysis for Graph Neural Networks}
\label{sec:GNN}
\label{sec:archvision}




\indent \textbf{Throughput plots for Graph Neural Networks:~} We evaluate GCN for SRAM size of 1MB as~\autoref{fig:GNN}a shows. Cora has a large feature matrix $M\times N$ but still has low arithmetic intensity due to low number of non zeros per row. There is a marginal improvement in \DataflowNamenospace -\textsc{Qpad} but considerable improvement with pipelining and hits the ideal. Protein dataset is relatively small and the tensors fit in the SRAM, thus both \DataflowNamenospace -\textsc{Qpad} and \DataflowNamenospace -\textsc{all} hit the ideal. Graph Neural Network layers do not have downstream tensors using the same data thus pipelining makes it easier to achieve the ideal DRAM accesses. Adjacent pipeline also achieves equal throughput as \DataflowNamenospace -\textsc{all} due to adjacent pipeline opportunities without delayed dependencies.

\textbf{Throughput plots for ResNet and SSD ResNet:} ~\autoref{fig:GNN}b and c show throughput plots for ResNets and SSD-ResNets. They always hit the peak being compute bound (\autoref{fig:roofline}). Thus pipelining is not helpful for performance, but can potentially help reduce energy, as we discuss next.

\textbf{DRAM access reduction}:~\autoref{fig:comm}a shows the DRAM access reduction across various applications. The adjacent pipeline baseline shows major reduction in DRAM accesses in all applications except CG due to delayed dependencies.
For ResNet and SSD-ResNet,
\DataflowNamenospace-\textsc{All} leads to additional reduction in DRAM accesses because of the ability to pipeline\textunderscore with\textunderscore hold as~\autoref{fig:buffer} shows. %\TK{@Raveesh - point back to Figure with ResNet pipeline with hold and remind that adj pipeline wont pipeline that}. 
Also, between ~\DataflowNamenospace-\textsc{Qpad} and adjacent pipelining, adjacent pipelining is better in case of SSD-ResNets and GNNs as~\DataflowNamenospace-\textsc{Qpad}'s benefit diminishes with larger working sets. However, in CG, adjacent pipelining has no benefit, and in ResNet, the working set is small enough for ~\DataflowNamenospace-\textsc{Qpad} to fully reuse the activation on chip.
%This is because, between adjacent pipeline and \DataflowNamenospace-\textsc{Qpad}, the better dataflow depends on the amount of adjacent pipelining that can be done and on the working set size.
%\TK{Raveesh - pls elaborate on the above explanation .. didnt understand. can u explan why a large or small working set affects Qpad performance?}
 ~\DataflowNamenospace-\textsc{All}, combining both of these and more optimizations, has the best DRAM access reduction for all the workloads.


\indent %\reviewme{\textbf{Roofline plots for Attention Layers:~}
%We evaluate attention layers for SRAM size of 4MB as~\autoref{fig:bert} shows. For sequence length of 64, \DataflowNamenospace -\textsc{Qpad} achieves near ideal and \DataflowNamenospace -\textsc{all} achieve the ideal AI. Note that even though, the baseline intensity relatively high, \DataflowName would allow the substrate to have a lower memory bandwidth. With increase in B and L, the gap between Flexgon-like and ideal widens. For sequence length of 256, baseline achieves significantly lower portion of the ideal, while \DataflowNamenospace -\textsc{Qpad} near ideal AI and \DataflowNamenospace -\textsc{all} achieves the ideal in case of B=1 At B=4, L=256, the working set becomes too big for the SRAM, \DataflowNamenospace \textsc{all} still achieves 60\% of the ideal AI due to fusion of operations.}
%\subsubsection{DRAM accesses in Graph Neural Networks}:

% Considers best case for GOGETA-df and worst for GOGETA-map.}
%\vspace{-2mm}
\label{sec:comm}
\indent \textbf{Impact of tiling on scalability:~}
%Pipelining between two operations involves, communicating the data between the parts of the compute where the operations are mapped.
~\autoref{fig:comm}b shows inter-cluster link traversal for with and without the tiling consideration in KB's when considering pipelining between operations defined in line 4 and 5 of~\autoref{alg:cg_einsum}. As~\autoref{sec:tiling} shows, splitting the dominant rank makes the inter-cluster traversal independent of M. Workload can scale up considerably and the dimension that will scale is $M$. By changing these to intra-cluster traversals, \DataflowName and even adjacent pipelining can make better use of the high bandwidth NoC. This analysis can be extrapolated to distributed systems where the cross compute node bandwidth is even worse than inter-cluster bandwidth.

\textbf{Impact of Memory BW}: Limiting the memory bandwidth further affects the throughput of the memory bound region and it increases the AI required to hit the peak.~\autoref{fig:comm}c shows the throughput of FV1 with memory BW of 1000 and 250 GB/s. With memory BW=250 GB/s, the performance in the memory bound region is lower and \DataflowNamenospace-\textsc{All} performs better than \DataflowNamenospace-\textsc{Qpad} due to higher arithmetic intensity.



==> tables/backup.tex <==


\begin{scriptsize}

\begin{table*}[t!]
\begin{center}

    
\begin{scriptsize}
    %\vspace{-3mm}
  \center
  \caption{Performance of CG compared to Linpack (HPL) and Peak. Adapted from HPCG~\cite{hpcg2021}.} 
    \label{table:related}

  %\Rav{There is space for remarks too if needed}}
  %\TK{@Raveesh - by x do you mean you can do either s or t for that dimension? So does that mean each row is actually multiple datapoints? Thats confusing.}\Rav{It means that the datapoint that we choose for evaluation of that dataflow can have varaible tile sizes for dimension marked by X. S and T on the other hand mean that its NECESSARILY spatial or temporal}}
  \begin{tabular}{|l|l|l|l|l|l|l|l|}
    \hline
    \textbf{Type} & \textbf{Examples} & 
    \textbf{Intra-op} & \textbf{Adjacent} & \textbf{Delayed} & \textbf{Parallel} & \textbf{Tiling} & \textbf{DAG-level} \\ & & \textbf{reuse} & \textbf{op reuse} & \textbf{op reuse} & \textbf{Multicast} & \textbf{Dependencies} & \textbf{layout}
\\    \hline
Op-by-op & MAESTRO~\cite{kwon2019understanding}, GAMMA~\cite{kao2020gamma} &   \greencheck & \redcheck & \redcheck & Tiling and ordering only care about maximizing reuse within \\
& CoSA~\cite{cosa}, Interstellar~\cite{interstellar} & & & &  the operation. Suffers if individual operations are memory bound.\\
\hline
Adjacent &  OMEGA~\cite{omega}, FlashAttention~\cite{flashattention} & \greencheck & \greencheck & \redcheck & Tiling and ordering care about pipelining with adjacent consumers. \\ Pipelining & FLAT~\cite{flat}, TANGRAM~\cite{tangram} & & & & Helps if individual operations are memory bound. However, it only \\& & & & & works if the consumer doesn't have a delayed downstream consumer. \\ \hline
Generalized & \DataflowName & \greencheck & \greencheck & \greencheck & Generalized inter-op reuse introduces new considerations-\\
Inter-op & & & & & -Considers reuse within delayed downstream consumers.\\
reuse & & & & & -Ordering also ensures minimizing layout transformations.\\
& & & & & -Tiling also ensures that the inter-cluster communication is minimized\\
& & & & & -Custom scratchpad management strategy considers reuse of a tensor\\
& & & & & within the entire program and not just adjacent operations.
\\\hline
  \end{tabular}
\vspace{-5mm}
\end{scriptsize}
\end{center}

\end{table*}

\end{scriptsize}

==> tables/dataflow.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Reuse opportunities for GEMM dimensions. (Intra-phase dataflow) \TK{the goal of this table is nice but I think we could simplify it and make it similar to Table II. @Eric - put a new table in "intra-phase dataflow" sheet in our spreadsheet. Can you put that here?}} %\TK{@Eric - can we replace this / augment this with a figure simply showing a GEMM mapped over a simple 2D array in a WS manner and show multicast of MK matrix, and spatial reduction across K?}}
\begin{tabular}{|l|l|l|}
\hline
\textbf{Dataflow} & \textbf{\begin{tabular}[c]{@{}l@{}}Implication of \\ Loop Order\end{tabular}}                                           & \textbf{\begin{tabular}[c]{@{}l@{}}Implication of \\ Spatial Dimensions\end{tabular}}                                                                     \\ \hline
\{Ms Ns\} Kt      & \begin{tabular}[c]{@{}l@{}}Output (MN) stationary,\\ Inputs (MK) and \\ Weights (KN) stream \\ every cycle\end{tabular} & \begin{tabular}[c]{@{}l@{}}Spatial multicast of \\ Inputs and Weights every\\ cycle. Temporal reduction\\ of partial sums within \\ each PE.\end{tabular} \\ \hline
\{Ns Ks\} Mt      & \begin{tabular}[c]{@{}l@{}}Weight (KN) stationary,\\ Input (MK) streams\\ every cycle\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}Spatial multicast of \\ inputs every cycle. \\ Spatial reduction of partial \\ sums across PEs\end{tabular}                    \\ \hline
\{Ms Ks\} Nt      & \begin{tabular}[c]{@{}l@{}}Input (MK) stationary, \\ Weight (KN) streams \\ every cycle\end{tabular}                    & \begin{tabular}[c]{@{}l@{}}Spatial multicast of \\ weights every cycle. \\ Spatial reduction of partial \\ sums across PEs\end{tabular}                   \\ \hline
\end{tabular}
\label{tables:dataflow}
\end{table}

==> tables/dataflow_bk.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Reuse opportunities for GEMM dimensions. (Intra-phase dataflow) \TK{the goal of this table is nice but I think we could simplify it and make it similar to Table II. @Eric - put a new table in "intra-phase dataflow" sheet in our spreadsheet. Can you put that here?}} %\TK{@Eric - can we replace this / augment this with a figure simply showing a GEMM mapped over a simple 2D array in a WS manner and show multicast of MK matrix, and spatial reduction across K?}}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{7}{|c|}{\textbf{Spatial}}                                                                                                                                                    & \multicolumn{7}{c|}{\textbf{Temporal}}                                                                              \\ \hline
\multirow{2}{*}{\textbf{Dimension}} & \multicolumn{3}{c|}{\textbf{Coupling}}                       & \multicolumn{3}{c|}{\textbf{Reuse}}                                                  & \multirow{2}{*}{\textbf{Dimension}} & \multicolumn{3}{c|}{\textbf{Coupling}} & \multicolumn{3}{c|}{\textbf{Reuse}}  \\ \cline{2-7} \cline{9-14} 
                                    & \textbf{B}         & \textbf{A}         & \textbf{O}         & \textbf{B}                 & \textbf{A}                 & \textbf{O}                 &                                     & \textbf{B}  & \textbf{A}  & \textbf{O} & \textbf{B} & \textbf{A} & \textbf{O} \\ \hline
\multirow{2}{*}{\textbf{M}}         & \multirow{2}{*}{}  & \multirow{2}{*}{Y} & \multirow{2}{*}{Y} & \multirow{2}{*}{Multicast} & \multirow{2}{*}{}          & \multirow{2}{*}{}          & K                                   & Y           & Y           &            &            &            & Reduction  \\ \cline{8-14} 
                                    &                    &                    &                    &                            &                            &                            & N                                   & Y           &             & Y          &            & Multicast  &            \\ \hline
\multirow{2}{*}{K}                  & \multirow{2}{*}{Y} & \multirow{2}{*}{Y} & \multirow{2}{*}{}  & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{Reduction} & M                                   &             & Y           & Y          & Multicast  &            &            \\ \cline{8-14} 
                                    &                    &                    &                    &                            &                            &                            & N                                   & Y           &             & Y          &            & Multicast  &            \\ \hline
\multirow{2}{*}{N}                  & \multirow{2}{*}{Y} & \multirow{2}{*}{}  & \multirow{2}{*}{Y} & \multirow{2}{*}{}          & \multirow{2}{*}{Multicast} & \multirow{2}{*}{}          & M                                   &             & Y           & Y          & Multicast  &            &            \\ \cline{8-14} 
                                    &                    &                    &                    &                            &                            &                            & K                                   & Y           & Y           &            &            &            & Reduction  \\ \hline
\end{tabular}
\label{tables:dataflow}
\end{table*}

==> tables/dataflow_config2.tex <==
\begin{scriptsize}

\begin{table}[h!]
    
\begin{scriptsize}
\begin{center}

    %\vspace{-3mm}
  \center
  \caption{Dataflow Configurations} 
  \label{table:dataflow_config}
  \begin{tabular}{|l|l|}
    \hline
    \textbf{Config} & \textbf{Description}  \\
    \hline
    %Seq & $V\times F$ & $t_{AGG}+t_{CMB}$\\
    %\hline
%    SEQ-Inner & Op-by-op Dataflow with Inner Product\\ \hline
    Flexagon~\cite{flexagon}-like*   
 & Flexagon's flexible architecture can optimally map a single
    \\
   (Op-by-op) & op with any shape and sparsity. It achieves  the best possible \\ & single operation AI. All ops begin and end in DRAM.\\ 
    \hline
    Adjacent Pipelining & Considers adjacent pipelining where it is possible\\  & without writeback/hold. \\\hline
    GOGETA-\textsc{Qpad} & While this dataflow is still Sequential, it uses \textsc{Qpad} \\  (\textsc{Qpad} only) & scheme to write the data to SRAM until its full to read it  \\ & in the same order.\\\hline
  %  GOGETA-df & GOGETA dataflow with inter-op pattern~\autoref{alg:inter-op} \\\hline
  %  & and loop orders~\autoref{alg:looporder}.\\\hline
    GOGETA-all & This datapoint uses the complete suite of contributions: inter\\
    (Inter-op Mapping &-op reuse patterns (\autoref{sec:dataflows}), loop-order(\autoref{sec:loop}),tiling\\
    +\textsc{Qpad}+\textsc{FDpad}) & (\autoref{sec:tiling}) \& custom scratchpad management(\autoref{sec:tornado}). \\\hline
    Ideal (AI\textsubscript{best}) & Considers prefect inter-op reuse with infinite SRAM. (AI\textsubscript{best})\\\hline
%    GOGETA+org & GOGETA-map with optimal tensor allocation ~\autoref{sec:tornado}\\\hline
    
    %Total L2 capacity & 32MB\\ \hline
    %Total L3 capacity & 256MB\\ \hline
    
  \end{tabular}\end{center}

  *{While Flexagon proposes an accelerator for SpMSpM, we model Flexagon’s flexible NoC and microarchitecture which can run any single operation dataflow and model SpMM and \GEMM on it.}







 % \vspace{1mm}
%\vspace{-4mm}
\end{scriptsize}

\end{table}

\end{scriptsize}

==> tables/dataflow_config_bk.tex <==
\begin{scriptsize}
\begin{table}[h!]
    
\begin{scriptsize}
\begin{center}

    %\vspace{-3mm}
  \center
  \caption{Dataflow Configurations} 
  \label{table:dataflow_config}
    \vspace{-2mm}
\begin{tabular*}{|p{0.18\linewidth}|p{0.72\linewidth}|}
    \hline
    \textbf{Config} & \textbf{Description}  \\
    \hline
    %Seq & $V\times F$ & $t_{AGG}+t_{CMB}$\\
    %\hline
%    SEQ-Inner & Op-by-op Dataflow with Inner Product\\ \hline
    Flexagon~\cite{flexagon}-like*   
 & Flexagon's flexible architecture can optimally map a single (Op-by-op) operation with any shape and sparsity. It achieves  the best possible single operation AI. All ops begin and end in DRAM. Its the oracle operation-by-operation dataflow.\\
    \hline
    Adjacent Pipelining & It considers inter-operation pipelining between two consecutive operations when it is possible to apply (no delayed dependency). \reviewmehpca{We also consider tiling strategy proposed in~\autoref{sec:tiling}.}
      \\\hline
    GOGETA-\textsc{Qpad} & \DataflowNamenospace-\textsc{Qpad} does not consider pipelining, however, it writes the portion of the tensor that fits in the scratchpad in FIFO order proposed in~\autoref{sec:tornado} but does not consider distance/frequency based replacement. This ensures that parts of intermediate tensors that could fit, are still reused inside the SRAM.\\\hline
  %  GOGETA-df & GOGETA dataflow with inter-op pattern~\autoref{alg:inter-op} \\\hline
  %  & and loop orders~\autoref{alg:looporder}.\\\hline
    \DataflowNamenospace-\textsc{All} & \DataflowNamenospace-\textsc{all} uses all the contributions proposed. It uses the inter-op patterns proposed in~\autoref{sec:dataflows} and finds the individual loop orders which enable pipelining and avoid swizzle\_penalty proposed in~\autoref{sec:loop} and also uses the scratchpad management in~\autoref{sec:tornado}. It also uses scalable tiling strategy that reduces inter-cluster communication overhead proposed in~\autoref{sec:tiling}.ith infinite SRAM. (AI\textsubscript{best})\\\hline
    Ideal & Perfect reuse with infinte SRAM
    \\\hline
%    GOGETA+org & GOGETA-map with optimal tensor allocation ~\autoref{sec:tornado}\\\hline
    
    %Total L2 capacity & 32MB\\ \hline
    %Total L3 capacity & 256MB\\ \hline
    
  \end{tabular*}\end{center}

  *{While Flexagon proposes an accelerator for SpMSpM, we model Flexagon’s flexible NoC and microarchitecture which can run any single operation dataflow and model SpMM and \GEMM on it.}

\vspace{-3mm}





 % \vspace{1mm}
%\vspace{-4mm}
\end{scriptsize}

\end{table}

\end{scriptsize}

==> tables/eval_config.tex <==
\begin{scriptsize}
\begin{table}[h!]
  \centering
  \caption{Representative dataflow configurations for evaluation.}
  %\TK{@Raveesh - by x do you mean you can do either s or t for that dimension? So does that mean each row is actually multiple datapoints? Thats confusing.}\Rav{It means that the datapoint that we choose for evaluation of that dataflow can have varaible tile sizes for dimension marked by X. S and T on the other hand mean that its NECESSARILY spatial or temporal}}
  \label{tables:eval_config}
  \begin{tabular}{|l|l|}
    \hline
    \textbf{Dataflow Configuration} & \textbf{Description} \\ \textbf{Compact name below} & \\
    \hline
    Seq\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{t},V\textsubscript{x}G\textsubscript{x}F\textsubscript{x}) & Sequential dataflow \\ Seq-N\textsubscript{t} & Temporal Aggregation \\
    \hline
    Seq\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{s},V\textsubscript{x}G\textsubscript{x}F\textsubscript{x}) & Sequential dataflow \\ Seq-N\textsubscript{s} & Spatial Aggregation\\
    \hline
    SP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{s}N\textsubscript{t},V\textsubscript{x}F\textsubscript{s}G\textsubscript{x}) & Sequential Pipeline dataflow \\ SP-F\textsubscript{s}N\textsubscript{t}-F\textsubscript{s}  & EnGN-like \\ & Temporal Aggregation\\ & Relatively high T\textunderscore F \\
    \hline
    %SP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{s}N\textsubscript{s},V\textsubscript{x}F\textsubscript{s}G\textsubscript{x}) & SP-F\textsubscript{s}N\textsubscript{s}-F\textsubscript{s} & Sequential Pipeline dataflow \\ & & Spatial Aggregation\\ & & Relatively high T\textunderscore F \\
    %\hline
    SP\textsubscript{AC}(V\textsubscript{s}F\textsubscript{x}N\textsubscript{t},V\textsubscript{s}F\textsubscript{x}G\textsubscript{x}) & Sequential Pipeline dataflow \\ SP-V\textsubscript{s}N\textsubscript{t}-V\textsubscript{s}  & EnGN-like \\ & Temporal Aggregation\\ & Relatively high T\textunderscore V \\
    \hline
    %SP\textsubscript{AC}(V\textsubscript{s}F\textsubscript{x}N\textsubscript{t},V\textsubscript{s}F\textsubscript{x}G\textsubscript{x}) & SP-V\textsubscript{s}N\textsubscript{s}-V\textsubscript{s} & Sequential Pipeline dataflow \\ & & Spatial Aggregation\\ & & Relatively high T\textunderscore V \\
    %\hline
    PP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{t},V\textsubscript{x}G\textsubscript{x}F\textsubscript{x}) & Parallel Pipeline dataflow \\ PP-N\textsubscript{t}-V\textsubscript{t/sl} & Temporal Aggregation\\ & HyGCN-like \\& Granularity of lower rows \\
    \hline
    PP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{s},V\textsubscript{x}G\textsubscript{x}F\textsubscript{x}) & Parallel Pipeline dataflow \\ PP-N\textsubscript{s}-V\textsubscript{t/sl} & Spatial Aggregation \\ & Granularity of lower rows \\
    \hline
    PP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{t},V\textsubscript{s}G\textsubscript{x}F\textsubscript{x})  & Parallel Pipeline dataflow \\ PP-N\textsubscript{t}-V\textsubscript{sh} & Temporal Aggregation\\ & HyGCN-like \\ &  Granularity of higher rows \\
    \hline
    PP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{s},V\textsubscript{s}G\textsubscript{x}F\textsubscript{x}) & Parallel Pipeline dataflow \\ PP-N\textsubscript{s}-V\textsubscript{sh}  & Spatial Aggregation\\ & Granularity of higher rows \\
    \hline
    SP{\textsubscript{AC}}(V{\textsubscript{s}}F{\textsubscript{x}}N{\textsubscript{t}},V{\textsubscript{s}}F{\textsubscript{x}}G{\textsubscript{x}})  & SP-V\textsubscript{s}N\textsubscript{t}-V\textsubscript{s} dataflow with \\ High-V{\textsubscript{s}}-SP & very high T\textunderscore V\\
    \hline
  \end{tabular}
\vspace{-3mm}
\end{table}
\end{scriptsize}

==> tables/geo.tex <==


\begin{scriptsize}

\begin{table}[h!]
\begin{center}

    
\begin{scriptsize}
    \vspace{-5mm}
  \center
  \caption{\reviewme{Dataset-wise Arithmetic Intensity gain in CG.}} 
    \label{tables:geo}

  %\Rav{There is space for remarks too if needed}}
  %\TK{@Raveesh - by x do you mean you can do either s or t for that dimension? So does that mean each row is actually multiple datapoints? Thats confusing.}\Rav{It means that the datapoint that we choose for evaluation of that dataflow can have varaible tile sizes for dimension marked by X. S and T on the other hand mean that its NECESSARILY spatial or temporal}}
\begin{tabular}{|l|l|l|l|l|}
    \hline
    \reviewme{\textbf{Dataset}} & \reviewme{nasa4704} & \reviewme{fv1} & \reviewme{shallow\textunderscore water1} & \reviewme{G2\textunderscore Circuit}  \\\hline
    \reviewme{\textbf{Gain}} & \reviewme{10.44x} & \reviewme{11.49x} & \reviewme{6.57x} & \reviewme{1.6x}
    \\\hline
  \end{tabular}
\vspace{-1mm}
\end{scriptsize}
\end{center}
\vspace{-5mm}
\end{table}

\end{scriptsize}

==> tables/intensity.tex <==
\begin{table*}[t!]
\begin{scriptsize}
\begin{center}
\caption{Arithmetic intensities of different sequences of Einsums with and without inter-operation reuse.}
{%\tt
\begin{tabular}{|r|c|c|c|}\hline
\textbf{Type} & \textbf{Einsum sequence} & \textbf{AI\textsubscript{best} without inter-operation reuse} & \textbf{AI\textsubscript{best} with inter-operation reuse} \\\hline
  & {$Z_{m,n}=\sum_{k}A_{m,k}*B_{k,n}$} &  & \\
  & {$Y_{o,n}=\sum_{j}C_{o,j}*Z_{j,n}$} & \begin{scriptsize} $MNK+ONM+PON+QPN+RQN$ \end{scriptsize}  & \begin{scriptsize} $MNK+ONM+PON+QPN+RQN$ \end{scriptsize} \\
 NN & {$X_{p,n}=\sum_{i}D_{p,i}*Y_{i,n}$} & ------------------------------------------------------------------------------------------ & ---------------------------------------------- \\
 like & {$W_{q,n}=\sum_{h}E_{q,h}*X_{h,n}$} & \begin{scriptsize} $MK+KN+2\times MN+OM+2\times ON+PO+2\times PN+QP+2\times QN+RQ+RN$ \end{scriptsize} & \begin{scriptsize} $MK+KN+OM+PO+QP+RQ+RN$ \end{scriptsize} \\
 & {$V_{r,n}=\sum_{g}F_{r,g}*W_{g,n}$} &  &   \\\hline
  & {$Z_{m,n}=\sum_{k}A_{m,k}*B_{k,n}$} &  & \\
  & {$Y_{o,n}=\sum_{j}C_{o,j}*Z_{j,n}$} & \begin{scriptsize} $MNK+4\times ONM$ \end{scriptsize} & \begin{scriptsize} $MNK+4\times ONM$ \end{scriptsize} \\
 HPC & {$X_{m,n}=\sum_{i}Z_{m,i}*Y_{i,n}$} & ----------------------------------------------------------------------------------- & ---------------------------------------------- \\
 like & {$W_{o,n}=\sum_{h}Y_{o,h}*X_{h,n}$} & \begin{scriptsize} $MK+KN+5\times MN+4\times OM+4\times ON$ \end{scriptsize} &  \begin{scriptsize} $MK+KN+OM+MN$ \end{scriptsize} \\
 & {$V_{m,n}=\sum_{g}X_{m,g}*W_{g,n}$}  &  &  \\\hline
 
\end{tabular}
}
\end{center}
\end{scriptsize}
\vspace{-0.35cm}

\label{table:ai}
\vspace{-0.15cm}
\end{table*}


==> tables/inter_equations.tex <==
\begin{table}[ht!]
\begin{scriptsize}

  \centering
  \caption{Runtime and buffering requirements for inter-phase dataflows}%\Rav{There is space for remarks too if needed}}
  %\TK{@Raveesh - by x do you mean you can do either s or t for that dimension? So does that mean each row is actually multiple datapoints? Thats confusing.}\Rav{It means that the datapoint that we choose for evaluation of that dataflow can have varaible tile sizes for dimension marked by X. S and T on the other hand mean that its NECESSARILY spatial or temporal}}
  \label{tables:inter_equations}
  \begin{tabular}{|l|l|l|}
    \hline
    \textbf{Inter-phase} & \textbf{Intermediate} & \textbf{Runtime}  \\
    \textbf{dataflow} & \textbf{Buffering} & \\
    \hline
    %Seq & $V\times F$ & $t_{AGG}+t_{CMB}$\\
    %\hline
    Seq & V$\times$F & t\textsubscript{AGG}+t\textsubscript{CMB}\\
    \hline
    SP-arbitrary & $Computed\_V\times$ & t\textsubscript{AGG}+t\textsubscript{CMB}\\
    & $Computed\_F$ & \\
    \hline
    %SP-EnGN-like & $0$ & $t_{AGG}+t_{CMB}-t_{load}$\\
    %\hline
    SP-EnGN-like & 0 & t\textsubscript{AGG}+t\textsubscript{CMB}-t\textsubscript{load}\\
    \hline
    %PP-Element & $2\times T\_V\times T\_F$ & \\
    %\hline
    PP-elements & 2$\times$T\textunderscore V\textsubscript{max}$\times$T\textunderscore F\textsubscript{max} & sum(max(t\textsubscript{AGG},\\ & & t\textsubscript{CMB})\textsubscript{PPel})\\
    \hline
   PP-Row & 2$\times$T\textunderscore V\textsubscript{max}$\times$F & sum(max(t\textsubscript{AGG},\\ & & t\textsubscript{CMB})\textsubscript{PPel})\\
    \hline
    PP-Column & 2$\times$V$\times$T\textunderscore F\textsubscript{max} & sum(max(t\textsubscript{AGG},\\ & & t\textsubscript{CMB})\textsubscript{PPel})\\
    \hline
  \end{tabular}
\vspace{-3mm}
\end{scriptsize}
\end{table}


==> tables/interleave.tex <==
\begin{table*}[ht!]
\scriptsize
\centering
\caption{Characterizing the design-space of dataflows for GNN Accelerators (Note that any direction will affect the aggregation and combination dimension variables, but similar concepts apply). Subscript s, t, x means spatial, temporal, either spatial or temporal respectively. Curly brackets '\{\}' show that the loop order is interchangeable.} %\TK{what is intermediate support? maybe change to  ``Intermediate Buffer". For the NoC/PE support for PP, are we direvtly sending dataa from PEs doing aggr to PEs doing comb? thats what explanation sounds like. If yes, why do we need Interm Buffer? If not, then the NoC field should be about writing values to interm buffer after aggr and reading from it during comb}\Rav{Yes, changed to "support to connect agg and cmb units to intermediate buffers"}} %\Rav{Me - SP and Seq done and expanded PP, should we keep all 3 rows of table for cmb->agg or compact that piece ? } %\TK{@Eric / Raveesh -- for PP, isnt there any specific requirement from NoC or PE wrt multicast or spatial reduction, depending on the dataflow? Depends on accelerator seems vague} \Rav{Actually it depends on tiles, how about "Temporal reduction requires in-place accumulation support and spatial dimesnions require multicast/spatial reduce"}\TK{Yeah but thats just a general statement. Can you mention in each row which dimensions requires multicast distribution, and which requires spatial or temporal reduction? Similar to Fig 3b. Also -- for the SP row, ``in-place buffers" is vague. Do you mean ``Requires support for storing outputs of the aggregation stage locally in the PEs so they can be reused as inputs for the combination stage" ? if yes, can you say that}
%\TODO{Need to specify what {}, x, s and t subscripts mean} %\TODO{Shorten 3rd row NoC multicast and PE support}}

\begin{tabular}{lllllll}
\toprule
\textbf{Inter Phase}                                                                      & \textbf{Aggregation} & \textbf{Combination} & \textbf{\begin{tabular}[c]{@{}l@{}}Intermediate \\ Buffer\end{tabular}} & \textbf{NoC / PE Support}                                                                                                             & \textbf{\begin{tabular}[c]{@{}l@{}}Example \& \\ Order\end{tabular}}      & \textbf{Remarks}                                                                                                                                                                                                                                                                                           \\
\toprule
\textbf{\begin{tabular}[c]{@{}l@{}}Sequential\\ (Seq)\end{tabular}}            & \{V\textsubscript{x} F\textsubscript{x} N\textsubscript{x}\}         & \{V\textsubscript{x} G\textsubscript{x} F\textsubscript{x}\}         & \multicolumn{1}{c}\cmark      & Depends on Accelerator                                                                                                               & \begin{tabular}[c]{@{}l@{}}TPU \cite{tpu-isca} \\ Eyeriss \cite{eyeriss2}\\ (any direction*)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Similar to running one full or tiled layer at a \\time. Outputs of one layer gets stored in \\scratchpad and rescheduled back into the PEs.\end{tabular}                                                                                                         \\ % \\
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Sequential\\ Pipeline \\ (SP)\end{tabular}} &  \{V\textsubscript{x} F\textsubscript{x}\} N\textsubscript{t}    & \{V\textsubscript{x} F\textsubscript{x}\} G\textsubscript{t}         & \multicolumn{1}{c}\xmark                                                                     & \begin{tabular}[c]{@{}l@{}}Requires support to\\ store phase 1 outputs \\locally inside PE, so \\ that phase 2 can use\\ them as inputs\end{tabular} & \begin{tabular}[c]{@{}l@{}}EnGN \cite{liang2020engn}\\ (any direction*)\end{tabular}          & \begin{tabular}[c]{@{}l@{}}No intermediate support required, as output data\\ of one phase is stationary in the buffers, and can \\ be used as input for the next phase. Order of V,F  \\ should be the same for both the phases. T\textunderscore V\textsubscript{AGG}=\\T\textunderscore V\textsubscript{CMB} and T\textunderscore F\textsubscript{AGG}=T\textunderscore F\textsubscript{CMB} and reduction\\ is temporal as data is always in in-place buffers. \end{tabular}                                                                                                   \\                      % \\
\hline
\textbf{}                                                                      & V\textsubscript{t} \{F\textsubscript{s} N\textsubscript{t}\}         & \{V\textsubscript{s} G\textsubscript{s} F\textsubscript{t}\}         &  \multicolumn{1}{c}\cmark        & \begin{tabular}[c]{@{}l@{}}Requires support to\\ store agg. phase outputs \\locally inside PE, so \\ that cmb. phase can use\\ them as inputs\end{tabular}                                                                                                        &     \begin{tabular}[c]{@{}l@{}}Rubik \cite{chen2020rubik} \\ (agg->cmb)\end{tabular}                                                                      & \begin{tabular}[c]{@{}l@{}} Paper also focuses on reducing redundant \\ aggregations by saving duplicate data onto a \\ private cache. Similar to EnGN, no intermediate \\ data reordering required  as output data of one \\ phase is stationary in PEs and is used as inputs \\ for the next phase. \end{tabular}                              

                                            \\      %                 \\
                                            \hline
\textbf{}                                                                      & \{V\textsubscript{x} F\textsubscript{x} N\textsubscript{x}\}         & \{V\textsubscript{x} G\textsubscript{x} F\textsubscript{x}\}         & \multicolumn{1}{c}\cmark       & 
\begin{tabular}[c]{@{}l@{}}Agg:V\textsubscript{s},F\textsubscript{s}  require multicast\\ distribution. N\textsubscript{s/t} requires\\ spatial/temporal reduction.\\ Cmb:V\textsubscript{s},G\textsubscript{s}  require multicast\\ distribution. F\textsubscript{s/t} requires \\ spatial/temporal reduction.  \end{tabular}  
&         (any direction*)                                                    & \begin{tabular}[c]{@{}l@{}}There will be a buffer/ setup delay between \\ aggregation and combination phases to remap\\ output data to new location.\end{tabular}     

\\                                                %    \\
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Parallel \\ Pipeline\\ (PP)\end{tabular}}   & \{V\textsubscript{x} F\textsubscript{x}\} N\textsubscript{x}         & \{V\textsubscript{x} F\textsubscript{x}\}  G\textsubscript{x}        & \multicolumn{1}{c}\cmark     & \begin{tabular}[c]{@{}l@{}}Need support to connect \\agg and cmb units to\\ intermediate buffer\end{tabular}                                                          & \begin{tabular}[c]{@{}l@{}}(agg -\textgreater cmb)\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Element(s) wise granularity}: Element(s) of the \\ intermediate matrix indexed by V,F can be \\ pipelined. The order of V,F should be same for \\ both phases. \end{tabular} \\ %\\ 
\hline

& V\textsubscript{x} \{F\textsubscript{x} N\textsubscript{x}\}         & V\textsubscript{x} \{G\textsubscript{x}  F\textsubscript{x}\}        & \multicolumn{1}{c}\cmark     & \begin{tabular}[c]{@{}l@{}}Need support to connect \\agg and cmb units to\\ intermediate buffer\end{tabular}                                                             & \begin{tabular}[c]{@{}l@{}}HyGCN \cite{yan2020hygcn} \\ DAC GNN \cite{Auten2020} \\ (agg -\textgreater cmb)\end{tabular} & \begin{tabular}[c]{@{}l@{}} \textbf{Row(s) wise granularity}: Row(s) of intermediate \\ matrix indexed by V can be pipelined. The order \\ should not be (VFN,VFG) since that can be done \\ element wise. HyGCN allocates fixed number of \\ PEs per unit, which may lead to stalls. E.g., \\combination engine idle while waiting. HyGCN  \\ dataflow - $PP_{AC}(V_x F_s N_t, V_s G_s F_t)$\end{tabular} \\ %\\
\hline
& F\textsubscript{x} \{V\textsubscript{x} N\textsubscript{x}\}         & F\textsubscript{x} \{G\textsubscript{x}  V\textsubscript{x}\}        & \multicolumn{1}{c}\cmark     & \begin{tabular}[c]{@{}l@{}}Need support to connect \\agg and cmb units to\\ intermediate buffer\end{tabular}                                                            & \begin{tabular}[c]{@{}l@{}}(agg -\textgreater cmb)\end{tabular} & \begin{tabular}[c]{@{}l@{}} \textbf{Column(s) wise granularity}: Column(s) of the \\ intermediate matrix indexed by F can be \\ pipelined. The order should not be (FVN,FVG).\end{tabular} \\ %\\
\hline
  & \{N\textsubscript{x} F\textsubscript{x}\} V\textsubscript{x}         & \{V\textsubscript{x} G\textsubscript{x}\}  F\textsubscript{x}        & \multicolumn{1}{c}\cmark    & \begin{tabular}[c]{@{}l@{}}Need support to connect \\agg and cmb units to\\ intermediate buffer\end{tabular}                                                            & \begin{tabular}[c]{@{}l@{}}(cmb -\textgreater agg)\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Element(s) wise granularity}: The order should \\be (NFV, VGF) or (FNV, GVF). V$\times$G matrix \\after cmb becomes N $\times$ F for agg. \end{tabular} \\ %\\
\hline
& N\textsubscript{x} \{V\textsubscript{x} F\textsubscript{x}\}         & V\textsubscript{x} \{G\textsubscript{x}  F\textsubscript{x}\}        & \multicolumn{1}{c}\cmark     & \begin{tabular}[c]{@{}l@{}}Need support to connect \\agg and cmb units to\\ intermediate buffer\end{tabular}                                                           & \begin{tabular}[c]{@{}l@{}} (cmb -\textgreater agg)\end{tabular} & \begin{tabular}[c]{@{}l@{}} \textbf{Row(s) wise granularity}: Order should not be \\(NFV, VGF) since it can be done element wise.\end{tabular} \\ %\\
\hline
& F\textsubscript{x} \{V\textsubscript{x} N\textsubscript{x}\}         & G\textsubscript{x} \{F\textsubscript{x}  V\textsubscript{x}\}        & \multicolumn{1}{c}\cmark     & \begin{tabular}[c]{@{}l@{}}Need support to connect \\agg and cmb units to\\ intermediate buffer\end{tabular}                                                             & \begin{tabular}[c]{@{}l@{}}AWB-GCN \cite{geng2019awb} \\ (cmb -\textgreater agg)\end{tabular} & \begin{tabular}[c]{@{}l@{}} \textbf{Column(s) wise granularity}: The order should \\ not be (FNV, GVF). AWB-GCN enables flexible \\ allocation of PEs for different phases to match \\ production and consumption rates. AWB-GCN  \\dataflow-
%$PP_{CA}(G_t F_t V_s, F_s N_t V_s)$ 
$PP_{CA}(F_s N_t V_s, G_t F_t V_s)$
\end{tabular}                                                                                                                           \tabularnewline \bottomrule                                              
\end{tabular}
\label{tables:interleave}
\vspace{-3mm}
\end{table*}

==> tables/interleave_bk.tex <==
\begin{table*}[]
\begin{tabular}{lllllll}
\textbf{Sequential}          & \{Vx, Fx, Nx\} & \{Vx, Gx, Fx\} & \begin{tabular}[c]{@{}l@{}}Buffer \& Data \\ Scheduler\end{tabular}                                                                            & \begin{tabular}[c]{@{}l@{}}NOC \& PEs requirement\\  depends on accelerator\end{tabular}                                                         & \begin{tabular}[c]{@{}l@{}}TPU, MAERI\\ (any direction)\end{tabular}                              & \begin{tabular}[c]{@{}l@{}}Similar to running one full or tiled layer at a time. Outputs of \\ one layer gets stored in S2 scratchpad / buffer and rescheduled\\ back into the PEs.\end{tabular}                                                                                                                                                                                                \\
\textbf{Sequential Pipeline} & \{Vs, Fs, Nt\} & \{Vs, Gs, Ft\} & \begin{tabular}[c]{@{}l@{}}None, output of one unit \\ is stationary in the PEs, \\ and can be used as input\\ for the next layer\end{tabular} & \begin{tabular}[c]{@{}l@{}}Requires in place\\ accumulation (so output \\ can be buffered inside PE\\ to use as inputs)\end{tabular}             & \begin{tabular}[c]{@{}l@{}}EnGN (comb --\textgreater agg)\\ (agg -\textgreater comb)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Agg. uses Fs if it is agg --\textgreater comb, and Gs if it is comb --\textgreater agg.\\ Interleaved is possible because the output of combination (V,G) matrix is stationary, \\ and the input to agg is also (V, G), which is also stationary!\\ for agg-\textgreater{}comb, may need circular buffer to stream in property bank (might be temporal)\end{tabular} \\
                             & \{Vx, Fx, Nx\} & \{Vx, Gx, Fx\} & Buffer \& Data Scheduler                                                                                                                       & \begin{tabular}[c]{@{}l@{}}NoC must be able to transfer\\ data to the corresponding\\ PEs (need 2 compute engine\\ or allocate PEs)\end{tabular} &                                                                                                   & will be a buffer/ setup in between aggregation and combination                                                                                                                                                                                                                                                                                                                                  \\
\textbf{Pipeline parallel}   & Vt, \{Fs, Nt\} & \{Vs, Gs, Ft\} & \begin{tabular}[c]{@{}l@{}}Buffer \& Data \\ Scheduler\end{tabular}                                                                            & \begin{tabular}[c]{@{}l@{}}Agg \& Comb both require\\ in place accumulation. Comb\\ Engine requires Store \& \\ Fwd links\end{tabular}           & HyGCN (agg -\textgreater comb)                                                                    & \begin{tabular}[c]{@{}l@{}}Has 'aggregation buffer and coordinator' between aggregation \& combination unit. \\ Fixed number of PEs per unit may lead to stalls between units.\\ Ex: combination engine idle, waiting for aggregation to finish\end{tabular}                                                                                                                                    \\
                             & \{Vs, Ft, Ns\} & \{Vs, Gt, Fs\} & Buffer \& Data Scheduler                                                                                                                       & \begin{tabular}[c]{@{}l@{}}Multicast NoC required\\ between PEs.\end{tabular}                                                                    & AWB-GCN (both ways)                                                                               & \begin{tabular}[c]{@{}l@{}}Authors looked into intra and Inter Layer pipelining. There is also flexible allocation\\ of PEs for different layers to match production and consumption rates.\end{tabular}                                                                                                                                                                                        \\
                             & \{Vx, Fx, Nx\} & \{Vx, Gx, Fx\} & Buffer \& Data Scheduler                                                                                                                       & \begin{tabular}[c]{@{}l@{}}NoC must be able to transfer\\ data to the corresponding\\ PEs (need 2 compute engine\\ or allocate PEs)\end{tabular} &                                                                                                   & Different dataflow and mappings --\textgreater different production and consumption rates                                                                                                                                                                                                                                                                                                      
\end{tabular}
\label{tables:interleavebk}
\end{table*}

==> tables/related.tex <==


\begin{scriptsize}

\begin{table*}[t!]
\begin{center}

    
\begin{scriptsize}
    %\vspace{-3mm}
  \center
  \caption{Scope of this work against prior work. Tiling Dependencies arise in case of inter-operation reuse since the producer-consumer communication happens on a tile by tile basis. Swizzle minimization ensures that loop orders are allocated such that, tensor's layout transformation is minimized.
  %\TK{reminder: multi-row for reuse approach}
} 
    \label{table:related}
  %\Rav{There is space for remarks too if needed}}
  %\TK{@Raveesh - by x do you mean you can do either s or t for that dimension? So does that mean each row is actually multiple datapoints? Thats confusing.}\Rav{It means that the datapoint that we choose for evaluation of that dataflow can have varaible tile sizes for dimension marked by X. S and T on the other hand mean that its NECESSARILY spatial or temporal}}
  \vspace{-3mm}
  \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
    \hline
    \textbf{Works} & \textbf{Reuse} & 
    \textbf{Intra-op} & \textbf{Adjacent} & \textbf{Delayed} & \textbf{Parallel} & \textbf{Tiling} & \textbf{Min} & \textbf{Scratchpad}&\textbf{Scope of} \\  & \textbf{Approach} & \textbf{reuse} & \textbf{op reuse} & \textbf{op reuse} & \textbf{Multicast} & \textbf{Dependencies} & \textbf{Swizzle}& \textbf{Mgmt for DAG}& \textbf{tensor's reuse}
\\    \hline
GAMMA-MAESTRO~\cite{kao2020gamma,kwon2019understanding}  & Op-by-op &  \greencheck & \redcheck & \redcheck & \redcheck & \redcheck & \redcheck & \redcheck & Within the \\
 CoSA~\cite{cosa}, Interstellar~\cite{interstellar} & & & & & & & &&same layer\\
\hline
  OMEGA~\cite{omega}, FlashAttention~\cite{flashattention} & Adjacent & \greencheck & \greencheck & \redcheck & \redcheck & \greencheck & \redcheck & \redcheck & Same+adjacent \\   FLAT~\cite{flat}, TANGRAM~\cite{tangram} & Pipelining & & & & & & && layers\\ \hline
   Inter-layer scheduling space & Adjacent & \greencheck & \greencheck & \redcheck & \greencheck & \greencheck & \redcheck & \redcheck &Same+adjacent+\\  definition~\cite{isca-pip} & Pipelining & & & & & & &&branching layers\\ \hline
 \DataflowName (This work) & Generalized & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck & \greencheck &  Within the\\
 & Inter-op reuse & & & & & &&&whole DAG
\\\hline
  \end{tabular}
\vspace{-5mm}
\end{scriptsize}
\end{center}

\end{table*}

\end{scriptsize}
